On the Kottwitz conjecture for local shtuka spaces

Kottwitz's conjecture describes the contribution of a supercuspidal represention to the cohomology of a local Shimura variety in terms of the local Langlands correspondence. A natural extension of this conjecture concerns Scholze's more general spaces of local shtukas. Using a new Lefschetz-Verdier trace formula for v-stacks, we prove the extended conjecture, disregarding the action of the Weil group, and modulo a virtual representation whose character vanishes on the locus of elliptic elements. As an application, we show that for an irreducible smooth representation of an inner form of $\mathrm{GL}_n$, the $L$-parameter constructed by Fargues-Scholze agrees with the usual semisimplified parameter arising from local Langlands.

==> LefschetzVerdier.tex <==
%\documentclass[11pt]{article}
%\usepackage{macros, xcolor}



%\begin{document}
%\maketitle

\section{The Lefschetz-Verdier trace formula for v-stacks}
\label{SectionLefschetzVerdier}

The goal of this section is to build up some machinery related to the Lefschetz-Verdier trace formula.

We briefly review the setup in the context of a separated finite type morphism of schemes $p\from X\to \Spec k$, where $k$ is an algebraically closed field.   Let $\ell$ be a prime unequal to the characteristic of $k$, and let $A$ be an object of $D(X_{\et},\overline{\Q}_\ell)$, the derived category of \'etale $\overline{\Q}_\ell$-sheaves on $X$.  Suppose $f\from X\to X$ is a $k$-linear endomorphism.  If we are given the additional datum of a morphism\footnotemark $Rf_!A\to A$,  we obtain an operator $Rp_!A\isom Rp_!Rf_!A\to Rp_!A$ on the compactly supported cohomology $Rp_!A=R\Gamma_c(X,A)$.
%
\footnotetext{Equivalently, a morphism $A\to Rf^!A$.  A special case occurs when $f$ is an automorphism, $A$ is an honest sheaf on $X_{\et}$,  and $A\to f^*A$ is a morphism, such as the identity morphism on the constant sheaf $A=\overline{\Q}_\ell$.  More generally, we may replace $f$ with an algebraic correspondence $c=(c_1,c_2)\from C\to X\times_k X$.  In that setting, the required extra datum is a morphism $c_1^*\mc{F} \to c_2^!\mc{F}$:  this is the notion of a {\em cohomological correspondence} lying over $c$.}

In the special case that $X$ is proper over $k$,  so that $R\Gamma_c(X,A)=R\Gamma(X,A)$, the Lefschetz-Verdier trace formula \cite{SGA5}, \cite{VarshavskyLefschetz} expresses $\tr (f\vert R\Gamma(X,A))$ in terms of data living on the fixed point locus $\Fix(f)$ of $f$.   In particular, at isolated fixed points $x\in \Fix(f)$, there are local terms $\loc_x(f,A) \in \overline{\Q}_\ell$, and if all fixed points are isolated, then $\tr (f\vert R\Gamma(X,A))$ is the sum of the $\loc_x(f,A)$.  

In order to apply the Lefschetz-Verdier trace formula, we need to assume that $A$ satisfies a suitable finiteness hypothesis (constructible of finite Tor dimension).   Under this hypothesis one establishes an isomorphism \cite[Expos\'e III,  (3.1.1)]{SGA5}
\begin{equation}
\label{EqCrucialIsomorphismSchemes}
 \D A \boxtimes_k^{\LL} A \isom \RHom(\pr_1^*A, \pr_2^!A) 
 \end{equation}
 in $D((X\times_k X)_{\et},\overline{\Q}_\ell)$,  where $\pr_1,\pr_2\from X\times_k X\to X$ are the projection maps, and $\D$ is Verdier duality relative to $k$.  Once \eqref{EqCrucialIsomorphismSchemes} is established, the definition of local terms and the validity of the Lefschetz-Verdier trace formula can be derived by applying Grothendieck's six functor formalism.    The special case where $X=\Spec k$ is instructive;  the finiteness condition on $A$ is that it be a perfect complex of $\overline{\Q}_\ell$-vector spaces,  and then \eqref{EqCrucialIsomorphismSchemes} reduces to the fact that $A^\vee\otimes^{\LL} A\to \operatorname{RHom}(A,A)$ is an isomorphism.   This allows us to express the trace of an endomorphism $f\in \End A$ as the image of $f$ under the evaluation map $A^\vee\otimes^{\LL} A\to \overline{\Q}_\ell$.  

In this section we extend the Lefschetz-Verdier trace formula to the setting of perfectoid spaces, diamonds, and v-stacks.   The main result is Theorem \ref{ThmLefschetzVerdier} and its corollary \eqref{EqLefschetzProperDiamonds}.  We very closely follow the formalism of \cite{LuZheng} concerning the symmetric monoidal 2-category of cohomological correspondences.   In both the schematic and perfectoid settings, the finiteness condition required of the object $A$ can be stated in terms of the property of {\em universal local acyclicity} (ULA);  as noted in \cite[Theorem IV.2.24]{FarguesScholze}, this is precisely the hypothesis necessary to obtain the isomorphism in \eqref{EqCrucialIsomorphismSchemes}.  

The statement of Lefschetz-Verdier is formally identical between the scheme and perfectoid settings.   But in the perfectoid setting, there arises the possibility that the fixed point locus $\Fix(f)$ has the structure of a locally profinite set, in which case the local terms appearing in Lefschetz-Verdier are not a function on $\Fix(f)$, but rather a {\em distribution} on $\Fix(f)$.  This observation is critical to our applications.  

For our applications, we have included two additional theorems concerning local terms in the perfectoid setting, which could also have been stated in the schematic setting and may be of independent interest.  Theorem \ref{ThmKunnethForCharacteristicClass} is a sort of K\"unneth isomorphism for local terms on a fiber product of stacks.   Theorem \ref{ThmCharClassOnXModG} states that in the situation of a smooth group $G$ acting on a diamond $X$,  the local terms corresponding to individual elements $g\in G$ agree with local terms computed on the quotient stack $[X/G]$.  


\subsection{Small v-stacks and the six-functor formalism}

We recall here some material from \cite{ScholzeEtaleCohomology} on the main classes of geometric objects we deal with:  perfectoid spaces, diamonds, and v-stacks.
Let $\Perf$ be the category of perfectoid spaces in characteristic $p$.  There are four topologies we consider on $\Perf$, which we list from coarsest to finest:  the analytic topology, the \'etale topology, the pro-\'etale topology, and the v-topology.  

The v-topology is a rough analogy for the fpqc topology on schemes.  All representable presheaves on $\Perf$ are sheaves for the v-topology \cite[Theorem 1.2]{ScholzeEtaleCohomology}.  

A {\em diamond} is a pro-\'etale sheaf on $\Perf$ of the form $X/R$, where $X$ is a perfectoid space and $R\subset X \times X$ is a pro-\'etale equivalence relation.  Diamonds are automatically v-sheaves \cite[Proposition 11.9]{ScholzeEtaleCohomology}.  A particularly well-behaved class of diamonds are the locally spatial diamonds \cite[Definition 1.4] {ScholzeEtaleCohomology}.  There is a natural functor $X\mapsto X^\diamond$ from analytic adic spaces over $\Z_p$ to locally spatial diamonds.  

A v-sheaf $Y$ on $\Perf$ is {\em small} if there exists a surjective map $X\to Y$ from a perfectoid space $X$.  A {\em small v-stack} \cite[Definition 12.4]{ScholzeEtaleCohomology} is a v-stack $Y$ on $\Perf$ such that there exists a surjective map $X\to Y$ from a perfectoid space, such that $X\times_Y X$ is a small v-sheaf.  

Let $\Lambda$ be a ring which is $n$-torsion for some $n$ prime to $p$.  For every v-stack $X$ there is a triangulated category $D_{\et}(X,\Lambda)$ \cite[Definition 1.7]{ScholzeEtaleCohomology}.  If $X$ is a locally spatial diamond, then $D_{\et}(X,\Lambda)$ is equivalent to the left-completion of the derived category of sheaves of $\Lambda$-modules on the \'etale topology of $X$ \cite[Proposition 14.15]{ScholzeEtaleCohomology}.

The familiar six functors of Grothendieck have analogues in the world of small v-stacks \cite[Definition 1.7]{ScholzeEtaleCohomology}.  There is a derived tensor product $\otimes_\Lambda^\LL$ and a derived internal hom $\RHom_{\Lambda}$.  For any morphism $f\from Y\to X$ of small v-stacks, there is a pair of adjoint functors $f^*$ and $Rf_*$.  

We propose for convenience the following definition. 

\begin{dfn} A morphism $f\from Y\to X$ is {\em representable in nice diamonds} or simply {\em nice} if is compactifiable \cite[Definition 22.2]{ScholzeEtaleCohomology}, representable in locally spatial diamonds \cite[Definition 13.3]{ScholzeEtaleCohomology}, and of locally finite geometric transcendence degree \cite[Definition 22.2]{ScholzeEtaleCohomology}.  
\end{dfn}

If $f\from Y\to X$ is representable in nice diamonds, then there are an adjoint pair of functors $Rf_!$ and $Rf^!$ \cite[Sections 22 and 23]{ScholzeEtaleCohomology}.  

\begin{thm}[{\cite[Theorem 1.8]{ScholzeEtaleCohomology}}]
\label{ThmSixOperations} The six operations $\otimes_\Lambda$, $\RHom_\Lambda$, $f^*$, $Rf_*$, $Rf_!$, and $Rf^!$ obey the rules:
\begin{enumerate}
\item[(P1.)]$f^*A \otimes_\Lambda^\LL f^*B \isom f^*(A\otimes_\Lambda^\LL B)$,
\item[(P2.)] $Rf_*\RHom_\Lambda(f^*A,B)\isom \RHom_\Lambda(A,Rf_*B)$,
\item[(P3.)] $Rf_!(A\otimes_\Lambda^\LL f^*B)\isom Rf_!A\otimes_\Lambda^\LL B$ (the projection formula),
\item[(P4.)] $\RHom_\Lambda(Rf_!A,B)\isom Rf_*\RHom_\Lambda(A,Rf^!B)$ (local Verdier duality),
\item[(P5.)] $Rf^!\RHom_\Lambda(A,B)\isom \RHom_\Lambda(f^*A,Rf^!B)$
\end{enumerate}
\end{thm}

We also need the following base change results.

\begin{thm}[{\cite[Theorem 1.9]{ScholzeEtaleCohomology}}]
\label{ThmBaseChange}
Let 
\begin{equation}
\label{EqCartesianDiagram}
\xymatrix{
Y' \ar[r]^{\tilde{g}} \ar[d]_{f'} & Y \ar[d]^f \\
X' \ar[r]_g & X 
}
\end{equation}
be a cartesian diagram of small v-stacks.
\begin{enumerate}
\item[(BC1.)] If $f$ is representable in nice diamonds, then $g^*Rf_! \isom Rf'_!\tilde{g}^*$.
\item[(BC2.)] If $g$ is representable in nice diamonds, then $Rg^!Rf_*\isom Rf_*'R\tilde{g}^!$. 
\end{enumerate}
\end{thm}

There is a notion of {\em cohomological smoothness} \cite[Definition 23.8]{ScholzeEtaleCohomology} for morphisms between v-stacks which are representable in nice diamonds.   Let $\Lambda$ be an $n$-torsion ring for some $n$ not divisible by $p$.  For a morphism $f\from Y\to X$ of small v-stacks which is representable in nice diamonds, there is a natural map of functors
\begin{equation}
\label{EqPullbackToUpperShriek}
Rf^!\Lambda_X\otimes_\Lambda^{\LL} f^*\to Rf^!,
\end{equation}
adjoint to 
\[Rf_!(Rf^!\Lambda_X \otimes^{\LL}_{\Lambda} f^*A) \stackrel{(P3)}{\isomto} Rf_!Rf^!\Lambda_X \otimes^{\LL}_{\Lambda} A \stackrel{\text{counit}}{\to} A.\]  If $f$ is cohomologically smooth, then \eqref{EqPullbackToUpperShriek} is an equivalence \cite[Theorem 1.10]{ScholzeEtaleCohomology}.  Furthermore, the object $Rf^!\Lambda_X$ is invertible in the monoidal category $D_{\et}(Y,\Lambda)$.  (For $X$ a small v-stack, an object $A$ of $D_{\et}(X,\Lambda)$ is invertible if and only if \'etale-locally on $X$ there is an isomorphism $A\isom \Lambda_X[n]$.)

There is also the following base change theorem involving cohomologically smooth morphisms.

\begin{thm}[{\cite[Theorem 1.10]{ScholzeEtaleCohomology}}] \label{ThmSmoothBaseChange}
In the cartesian diagram \eqref{EqCartesianDiagram}, assume that $f$ is cohomologically smooth.  Then $\tilde{g}^*Rf^!\isom R(f')^!g^*$ and $(f')^*Rg^!\isom R\tilde{g}^! f^*$.  
\end{thm}


Finally, we need the notion of the dualizing complex for v-stacks.

\begin{dfn}[The dualizing complex]  Let $f\from X\to S$ be a morphism of small v-stacks which is representable in nice diamonds.  We define $K_{X/S}=Rf^!\Lambda$, an object in $D_{\et}(X,\Lambda)$.  

Suppose we are in the special case that $S=\Spd C$ for an algebraically closed perfectoid field $C$, and that $f$ is proper.  Then $Rf_*=Rf_!$, and so there is a morphism $Rf_*K_{X/S}=Rf_!Rf^!\Lambda \overset{\mathrm{counit}}{\longrightarrow} \Lambda$, which induces a morphism on the level of global sections
\[ H^0(X,K_{X/S})=H^0(S,Rf_*K_{X/S})\to H^0(S,\Lambda)=\Lambda, \]
which we notate as $\omega\mapsto \int_X \omega$.  
\end{dfn}



We record the following lemmas for convenience.
\begin{lem} 
\label{LemInvertibleSheaf}
Let $f\from Y\to X$ be a nice morphism of $S$-Artin v-stacks, and let $A,I\in D_{\et}(X,\Lambda)$ with $I$ invertible.  The natural map $Rf^!A\otimes^{\LL}_{\Lambda} f^*I \to Rf^!(A\otimes I)$ of \eqref{EqPullbackToUpperShriek} is an isomorphism.
\end{lem}

\begin{proof} Let $w_{A,I}$ be this morphism.  We also get a map $w_{A\otimes I,I^{-1}}\from Rf^!(A \otimes^{\LL}_{\Lambda} I) \otimes f^*I^{-1} \to Rf^!A$, which induces $Rf^!(A\otimes I)\to Rf^!A \otimes f^*I$.  This is the inverse to $w_{A,I}$.
\end{proof}


\begin{lem}  \label{LemTrivialDualizingSheaf} Let $f\from Y\to X$ be a morphism of $S$-Artin v-stacks which is cohomologically smooth.  There is a canonical isomorphism
\begin{equation}
\label{EqInverseDualizingComplexes}
R\Delta_{Y/X}^!\Lambda_{Y\times_X Y} \otimes^{\LL}_{\Lambda} Rf^!\Lambda_X \isom \Lambda_Y,
\end{equation}
so that $K_{Y/Y\times_X Y} \isom K_{Y/X}^{-1}$ is invertible.  
\end{lem}

\begin{proof} Let $\pr_1,\pr_2\from Y\times_X Y\to Y$ be the projection morphisms;  each is cohomologically smooth.  We have 
\[\Lambda_Y\isom R\id_Y^!\Lambda_Y\isom R\Delta_{Y/X}^!R\pr_1^!\Lambda_Y \isom R\Delta_{Y/X}^!\Lambda_{Y\times_X Y} \otimes^{\LL}_{\Lambda} \Delta_{Y/X}^*R\pr_1^!\Lambda_Y,\]
where in the last isomorphism we used Lemma \ref{LemInvertibleSheaf} combined with the cohomological smoothness of $R\pr_1$.  Now use Theorem \ref{ThmSmoothBaseChange} to obtain an isomorphism $\Delta_{Y/X}^*R\pr_1^!f^*\Lambda_X \isom \Delta_{Y/X}^*\pr_2^*Rf^!\Lambda_X\isom Rf^!\Lambda_X$.
\end{proof}

For the remainder of the section,  we fix $\Lambda$, an $n$-torsion ring for some $n$ not divisible by $p$.  We will now start writing $f_!$ for $Rf_!$ and $\otimes$ for $\otimes^{\LL}_{\Lambda}$, etc.


%\subsection{The ULA property}
%
%Let $f\from X\to S$ be a morphism of small v-stacks which is representable in nice diamonds.  Let $A\in D_{\et}(X,\Lambda)$.   There is a property of $A$ being {\em universally locally acyclic} (ULA) with respect to $f$ \cite[Definitions IV.2.1 and IV.2.23]{FarguesScholze}.  There is an equivalent formulation of this property, which will be very useful for proving a Lefschetz trace formula.
%
%\begin{thm}[{\cite[Theorem IV.2.24]{FarguesScholze}}] 
%\label{ThmULAEquivalence}
%Let $X\to S$ be a small v-stack which is representable in nice diamonds, and let $A\in D_{\et}(X,\Lambda)$.  The following are equivalent.
%\begin{enumerate}
%\item The complex $A$ is f-ULA.
%\item The natural map
%\[ \D_{X/S}A \boxtimes_S^{\LL} A \to \RHom_\Lambda(\pr_1^* A,R\pr_2^!A)\]
%is an isomorphism, where $\pr_1,\pr_2\from X\times_S X\to X$ are the two projections.
%\end{enumerate}
%\end{thm}
%
%\begin{exm}  In the case that $X=S=\Spd C$ for an algebraically closed perfectoid field $C$, we may identify $D_{\et}(X,\Lambda)$ with the derived category of $\Lambda$-modules.  Theorem \ref{ThmULAEquivalence} says that $A$ is ULA with respect to the identity on $\Spd C$ if and only if the natural map $\RHom(A,\Lambda[0])\otimes^{\LL}_{\Lambda} A \to \RHom(A,A)$ is an isomorphism.  This is true if and only if $A$ is a perfect complex, cf. Lemma \ref{lem:reflexivemodules}. 
%\end{exm}

%The ULA property is stable under proper pushforwards and smooth pullbacks in many contexts.  (These results are stated in \cite{FarguesScholze} in the setting where $S$ is a diamond, but they still hold for general small v-stacks $S$, cf. the comment preceding \cite[Definition IV.2.23]{FarguesScholze}.)



%not sure if we really need these.
%\begin{thm}[{\cite[Proposition IV.2.11]{FarguesScholze}}] 
%\label{ThmProperPushforward}
%Let $g\from Y\to X$, $f\from X\to S$ be maps of locally spatial diamonds.  Assume that $g$ is proper and that $f$ is compactifiable, and that both maps locally have finite geometric transcendence degree.  Assume that $A\in D_{\et}(Y,\Lambda)$ is $f\circ g$-ULA.  Then $Rg_*A\in D_{\et}(X,\Lambda)$ is $f$-ULA.  
%\end{thm}
%
%\begin{pro}[{\cite[Proposition IV.2.13]{FarguesScholze}}]
%\label{ProSmoothPullback} Let $f\from X\to S$ be a map of v-stacks which is representable in nice diamonds.  Let $g\from Y\to X$ be cohomologically smooth.  If $A\in D_{\et}(X,\Lambda)$ is ULA over $S$, then so is $g^*A$.
%\end{pro}


%\begin{pro}[{\cite[Proposition IV.2.19]{FarguesScholze}}] 
%Let $f\from X\to S$ be a morphism of small v-stacks which is representable in nice diamonds, and let $A\in D_{\et}(X,\Lambda)$ be ULA with respect to $f$.  Then for any $B\in D_{\et}(S,\Lambda)$, the natural map
%\[ \D_{X/S}(A)\otimes_\Lambda^\LL f^*B\to \RHom_\Lambda(A,Rf^!B) \]
%is an isomorphism.
%\end{pro}
%

%We will also need the following ``reflexivity'' properties for ULA objects.
%
%\begin{thm}[{\cite[Corollary IV.2.26]{FarguesScholze}}] 
%\label{ThmStrongReflexivity} Let $S$ be a small v-stack.
%\begin{enumerate}
%\item Let $f\from X\to S$ be representable in nice diamonds.  If $A\in D_{\et}(X,\Lambda)$ is $f$-ULA, then the biduality map 
%\[ A\to \D_{X/S}\D_{X/S} A \]
%is an isomorphism.  
%\item Let $f_i\from X_i\to S$ ($i=1,2$) be two morphisms of small v-stacks which are representable in nice diamonds.  Let $A_i\in D_{\et}(X_i,\Lambda)$ be $f_i$-ULA for $i=1,2$.  Then the natural map
%\[ \D_{X_1/S}A_1 \boxtimes_S \D_{X_2/S} \to \D_{X_1\times_S X_2} (A_1\boxtimes_S A_2) \]
%is an isomorphism.
%\end{enumerate}
%\end{thm}
%
%\begin{lem} Let $X_i\to S$ ($i=1,2$) be two morphisms of small v-stacks which are representable in nice diamonds.  Let $\pr_i\from X_1\times_S X_2\to X_i$ ($i=1,2$) be the projections.   Let $A_i\in D_{\et}(X_i,\Lambda)$ be ULA over $S$ for $i=1,2$.  Then we have an isomorphism in $D_{\et}(X_1\times_S X_2,\Lambda)$:
%\[ \D_{X/S}A_1\boxtimes_S A_2 \isom \RHom(\pr_1^*A_1,\pr_2^!A_2).\]
%\end{lem}
%
%\begin{proof}  We will describe a sequence of morphisms
%\begin{equation}
%\label{EqFourTermSequence}
%\D_{X_1/S}A_1 \boxtimes_S A_2 \to \RHom(\pr_1^*A_1,\pr_2^!A_2)\to \D_{X_1\times_S X_2}(A_1\boxtimes_S \D_{X_2/S}A_2) \to \RHom(\pr_1^*A_1,\pr_2^!A_2),
%\end{equation}
%in which the composition of the first two morphisms is the isomorphism of Theorem \ref{ThmStrongReflexivity}(ii), and the composition of the final two morphisms is the identity.  
%
%
%\end{proof}

%Now suppose $c\from Y\to X\times_S X$ is a morphism of small v-stacks over $S$ which is representable in nice diamonds.  Let $c_i=\pr_i\circ c$ for $i=1,2$.  We have an isomorphism
%\begin{equation}
%\label{EqRcUpperShriek}
%Rc^!(\D_{X/S}A\boxtimes_S^{\LL} A)
%\isom \RHom_\Lambda(c_1^*A,Rc_2^!A), 
%\end{equation}
%using Theorem \ref{ThmULAEquivalence} and (P5).  
%
%Let $\Delta_{X/S}\from X\to X\times_S X$ be the diagonal morphism.  Then $\Delta_{X/S}$ is also representable in nice diamonds [is this at all subtle??].  Let $\Fix(c)$ be the fixed point locus of the correspondence $c$, defined as the cartesian product
%\[
%\xymatrix{
%\Fix(c) \ar[r]^{c'} \ar[d]_{\Delta_{X/S}'} & X \ar[d]^{\Delta_{X/S}} \\
%Y \ar[r]_c & X 
%}
%\]
%Let $A\in D_{\et}(X,\Lambda)$.  The composition $\Delta_{X/S}^*(\D_{X/S}A \boxtimes_S^\LL A) = \D_{X/S}A \otimes_{\Lambda}^{\LL} A \to K_{X/S}$ induces by adjunction a morphism
%\begin{equation}
%\label{EqEvaluation}
%\D_{X/S}A \boxtimes_S^\LL A \to (\Delta_{X/S})_*K_{X/S}.
%\end{equation}
%
%\begin{dfn}[The trace morphism, and local terms] 
%\label{DfnTraceMorphism}
%Let $X\to S$ be a morphism of v-stacks which is representable in nice diamonds.  The trace morphism 
%\[ \underline{\tr}_c\from \RHom_{\Lambda}(A,A) \to 
%\]
%is defined as the composition:
%\begin{eqnarray*}
%\RHom_{\Lambda}(c_1^* A,Rc_2^! A) 
%&\stackrel{\label{EqRcUpperShriek}}{\isom}& 
%Rc^!(\D_{X/S}A \boxtimes^{\LL}_S A) \\
%&\stackrel{\eqref{EqEvaluation}}{\to}&
%Rc^!(\Delta_{X/S})_*K_{X/S} \\
%&\stackrel{\text{Thm.} \ref{ThmBaseChange}(2)}{\isom}&
%(\Delta'_{X/S})_*R(c')^! K_{X/S} \\
%&\isom& (\Delta'_{X/S})_* K_{\Fix(c)/S}.
%\end{eqnarray*}
%Let 
%\[ \tr_c\from \Hom_{\Lambda}(c_1^*A,Rc_2^!A) \to H^0(\Fix(c),K_{\Fix(c)/S}) \]
%be the morphism induced from $\underline{\tr}_c$ by taking global sections over $Y$.  Finally, we define local terms as follows, under the assumption that $S$ is connected.  For a morphism $u\from c_1^*A\to Rc_2^!A$, and an open and closed subset $\beta\subset \Fix(c)$ which the structure map $f_\beta\from \beta\to S$ is proper (so that $R(f_\beta)_*\isom R(f_\beta)_!$), let $\loc_\beta(u)\in \Lambda$ be the image of $\tr_c(u)\vert_\beta$ under
%\begin{eqnarray*}
%H^0(\beta,K_{\Fix(\beta)/S})
%&\isom& H^0(S,R(f_\beta)_*K_{\Fix(\beta)/S})\\
%&\isom& H^0(S,R(f_\beta)_!Rf_\beta^!\Lambda) \\ 
%&\stackrel{\text{counit}}{\to}& H^0(S,\Lambda)=\Lambda. 
%\end{eqnarray*}
%\end{dfn}
%
%\begin{exm} Suppose $X=S=\Spd C$, and let $c=c_1=c_2=\id_S$.  An object $A\in D_{\et}(S,\Lambda)$ which is ULA with respect to $\id_S$ is the same thing as a perfect complex.  An endomorphism $u\in \Hom_\Lambda(A,A)$ may be represented by a morphism of bounded complexes of $u^\bullet\from A^\bullet\to A^\bullet$, where each $A^i$ is a projective $\Lambda$-module.  Then $\tr_c(u)=\sum_i (-1)^i\tr(u^i)$.
%\end{exm}




\subsection{Artin v-stacks}

In our applications, we will encounter stacky maps $f\from Y\to X$ between v-stacks, for which $f_!$ and $f^!$ are not available using the material in \cite{ScholzeEtaleCohomology}.  In \cite{EnhancedSixFunctors}, the full six-functor formalism is extended to a class of stacky maps between Artin v-stacks, using the $\infty$-categorical machinery of \cite{LiuZheng}.  

%\begin{dfn}[{\cite[Definition IV.1.1]{FarguesScholze}}] \label{DfnDualizingComplexStacky} An {\em Artin v-stack} is a small v-stack $\mf{X}$ such that the diagonal $\Delta_{\mf{X}} \from \mf{X}\to \mf{X}\times \mf{X}$ is representable in locally spatial diamonds, and such that there is some surjective map $g\from U\to \mf{X}$ from a locally spatial diamond $U$ such that $g$ is separated and cohomologically smooth.
%\end{dfn}

\begin{dfn}[{\cite[Definition IV.1.1]{FarguesScholze}}] \label{DfnArtinVStack} An {\em Artin v-stack} is a small v-stack $X$ such that the diagonal $\Delta_X \from X\to X$ is representable in locally spatial diamonds, and such that there is some surjective map $g\from U\to X$ from a locally spatial diamond $U$ such that $g$ is separated and cohomologically smooth.  

A morphism of v-stacks $f\from Y\to X$ is {\em smooth-locally nice} if there exists a surjective cohomologically smooth map $g\from U\to Y$ from a locally spatial diamond $U$ such that $f\circ g$ is nice.  

Similarly we define for a fixed small v-stack $S$ the notion of an $S$-Artin v-stack $X \to S$, by requiring that the relative diagonal $\Delta_{X/S}\from X \to X \times_S X$ is representable in locally spatial diamonds.  
\end{dfn}

\begin{thm}[{\cite{EnhancedSixFunctors}}] If $f\from Y\to X$ is any smooth-locally nice map of Artin v-stacks, there exist functors $f_!$ and $f^!$ satisfying the properties listed in Theorems \ref{ThmSixOperations} and \ref{ThmBaseChange}, agreeing with the constructions in \cite{ScholzeEtaleCohomology} when $f$ is nice.  
\end{thm}

\begin{dfn}[{\cite[Definition IV.1.10]{FarguesScholze}}] \label{DfnCohomologicallySmoothStacky} Let $f\from Y\to X$ be a map of Artin v-stacks.  Then $f$ is {\em cohomologically smooth} if there exists a separated, representable in locally spatial diamonds, and cohomologically smooth surjection $g\from U\to Y$ from a locally spatial diamond such that $f\circ g\from U\to X$ is nice and cohomologically smooth.
\end{dfn}

%If $f\from \mf{X}\to S$ is a cohomologically smooth map of Artin v-stacks, then it is straightforward to define the dualizing complex $K_{\mf{X}/S}$.  Indeed, if $g\from U\to \mf{X}$ is a uniformization as in Definition \ref{DfnCohomologicallySmoothStacky}, then $K_{U/S}$ is an invertible object of $D_{\et}(U,\Lambda)$, which comes equipped with a descent datum along $U\to \mf{X}$.  Since $K_{U/S}$ is locally concentrated in a single degree, the descent datum is effective.  The result is that there is an invertible object $K_{\mf{X}/S}$ of $D_{\et}(\mf{X},\Lambda)$, equipped with 
%an isomorphism $Rg^!K_{\mf{X}/S}\isom K_{U/S}$ for any $g$ as in Definition \ref{DfnCohomologicallySmoothStacky}.  The data of $K_{\mf{X}/S}$ together with these isomorphisms is unique up to unique isomorphism. 
%
%%  We may also define the functor $Rf^!$ by $A\mapsto  Rf^!\Lambda\otimes_\Lambda^\LL f^*A$ \cite[Definition IV.1.14]{FarguesScholze}.  This functor admits a right adjoint $Rf_!$ \cite[Remark IV.1.15]{FarguesScholze}.
%
%We define here a more general class of stacky maps for which the dualizing complex exists.
%
%\begin{dfn} \label{DfnClassC} An $S$-Artin v-stack $f\from \mf{X}\to S$ is {\em of class $\mc{C}$} if there exists a separated and cohomologically smooth surjection $g\from U \to \mf{X}$, such that $f\circ g\from U\to S$ is representable in nice diamonds, and if $\Lambda_U$ is $(f\circ g)$-ULA.  
%\end{dfn}
%
%\begin{lem} Let $f\from \mf{X}\to S$ be a morphism of class $\mc{C}$ between Artin v-stacks.  Then a dualizing complex $K_{\mf{X}/S}$ exists and is unique up to unique isomorphism.   
%\end{lem}
%
%\begin{proof}  Given a uniformization $g\from U\to \mf{X}$ as in Definition \ref{DfnClassC}, we have the dualizing complex $K_{U/S}$, which comes equipped with a descent datum along $U\to \mf{X}$.  By the gluing lemma \cite[Theorem 3.2.4]{BBD}, the descent datum is effective so long as $\Ext^i_\Lambda(K_{V/S},K_{V/S})=0$ for all $i<0$, where $V$ is an $n$-fold product of $U$ over $\mf{X}$.  The resulting object $K_{\mf{X}/S}$  together with the isomorphisms $Rg_V^!K_{\mf{X}/S} \isom K_{V/S}$, is unique up to unique isomorphism;  this is the dualizing complex.  
%
%By hypothesis, $\Lambda_U$ is ULA over $S$.  By Proposition \ref{ProSmoothPullback}, $\Lambda_V$ is also ULA over $S$.  By Theorem \ref{ThmStrongReflexivity}, $\Lambda_V\isom \D_{V/S}\D_{V/S}\Lambda_V$, which is in turn isomorphic to  $\RHom(K_{V/S},K_{V/S})$.  Therefore $\Ext^i_\Lambda(K_{V/S},K_{V/S})\isom H^i(V,\Lambda_V)=0$ for $i<0$.
%\end{proof}




%\subsection{Inertia stacks and trace distributions}
%
%In this subsection we define the notion of the ``trace distribution'' of a complex $A$ on an Artin v-stack.  This is the stacky version of the local terms defined in Definition \ref{DfnTraceMorphism}.  
%
%We need the concept of the inertia stack \cite[\S8.7]{stacks-project}.
%
%\begin{dfn} Let $f\from \mf{X}\to S$ be a morphism of Artin v-stacks.  The {\em inertia stack} $\In_S(\mf{X})$ as the Cartesian product
%\[
%\xymatrix{
%\In_S(\mf{X}) \ar[r]^{h_{\mf{X}}} \ar[d]_{h_{\mf{X}}} & \mf{X}\ar[d]^{\Delta_{\mf{X}/S}} \\
%\mf{X} \ar[r]_{\Delta_{\mf{X}/S}} & \mf{X}\times_S \mf{X}
%}
%\]
%\end{dfn}
%Thus $\In_S(\mf{X})$ classifies pairs $(T,g)$, where $T$ is an object of $\mf{X}$ and $g\in \Aut_S T$.  It is also an Artin (v-)stack. 
%
%\begin{exm} \label{ExampleInertiaStack}  Let $\mf{X}=[X/G]$ for a diamond $X\to S$ admitting an $S$-linear action of a group diamond $G\to S$.  Then $\In_S(\mf{X})=[Y/G]$, where
%\[  Y=\set{(x,g)\in X\times G\biggm\vert g(x)=x}, \]
%and the action of $G$ on $Y$ is $h(x,g)=(hx,hgh^{-1})$.  In particular, $\In([S/G])=[G\stslash G]$ is the stack of conjugacy classes of $G$.
%\end{exm}
%
%
%
%
%\begin{dfn}[The trace distribution]
%\label{DfnTraceDistribution} Let $\mf{X}\to S$ be a morphism of  Artin v-stacks that admits a dualizing complex as in \ref{DfnDualizingComplexStacky}.  Let $A\in D_{\et}(\mf{X},\Lambda)$ be ULA over $S$.   Let $\trdist(A)\in H^0(\In_S(\mf{X}),K_{\mf{X}/S})$ be the image of the the identity morphism $A\to A$ under the composition
%\begin{eqnarray*}
%\RHom_\Lambda(A,A)
%&\stackrel{\text{Thm. }\ref{ThmSixOperations}(5)}{\isom}& R\Delta_{\mf{X}/S}^!\RHom_\Lambda(\pr_1^*A,\pr_2^!A) \\
%&\stackrel{\text{Prop. }\ref{ProCrucialIsomorphismStacky}}{\isom}& 
%R\Delta_{\mf{X}/S}^! (\D_{\mf{X}/S}A\boxtimes_S^{\LL} A) \\
%&\to& R\Delta_{\mf{X}/S}^! R(\Delta_{\mf{X}/S})_* (\D_{\mf{X}/S}A \otimes^{\LL} A) \\
%&\stackrel{\text{eval}}{\to}& R\Delta_{\mf{X}/S}^! R(\Delta_{\mf{X}/S})_* K_{\mf{X}/S} \\
%&\stackrel{\text{Thm. }\ref{ThmBaseChange}(2)}{\isom}& (Rh_{\mf{X}/S})_*(Rh_{\mf{X}/S})^! K_{\mf{X}/S} \\
%&\isom& (Rh_{\mf{X}/S})_*K_{\In_S(\mf{X})/S}. 
%\end{eqnarray*}
%\end{dfn}
%
%
%\begin{exm} Let $S=\Spd C$ for an algebraically closed perfectoid field $C$.  Let $G$ be a locally pro-$p$ group, such that $\mf{X}=[S/G_S]$ is a smooth Artin stack.   We consider an object $A$ of $D_{\et}(\mf{X},\Lambda)$ as a complex of  $\Lambda$-modules with smooth $G$-actions.  Then $A$ is ULA over $S$ if and only if it is admissible, in the sense that for all compact open subgroups $K\subset G$, the invariant complex $A^K$ is perfect.
%
%After choosing a Haar measure on $G$, we have (after Example \ref{ExampleGInvariantDistributions}) an isomorphism $H^0(\In_S(\mf{X}),K_{\In_S(\mf{X})/S})\isom \Dist(G,\Lambda)^G$ (conjugation-invariant $\Lambda$-valued distributions on $G$).  With respect to this isomorphism, $\trdist(A)$ is the trace distribution of $G$ on $A$.   (Explicitly:  if $f\in C_c(G,\Lambda)$ is a compactly supported smooth function, then it is bi-$K$-invariant for a compact open subgroup $K\subset G$, and then $\trdist(A)(f)$ equals the trace of integration against $f$ on $A^K$.
%\end{exm}



\subsection{The category of cohomological correspondences}

%In this subsection we show that formation of the trace distribution $\trdist A$ is compatible with proper pushforward.  The result will be a (relative) Lefschetz-Verdier trace formula.  This is the form of Lefschetz-Verdier that will be used to compute the cohomology of spaces of mixed-characteristic shtukas.  
%
%We assume throughout that either $S=\Spd k$ for a (discrete) algebraically closed perfect field $k$, or else $S=\Spd C$ for an algebraically closed perfectoid field $C$. 
%
%For a morphism $f\from \mf{X}\to Y$ of $S$-Artin v-stacks, let $\In_S(f)\from \In_S(\mf{X})\to\In_S(Y)$ be the associated morphism between $S$-inertia stacks.  
%
%\begin{thm} \label{ThmLefschetzVerdierStacky} {\color{red} Assume that the six-functor formalism described in Theorems \ref{ThmSixOperations} and \ref{ThmBaseChange} applies to all morphisms bertween $S$-Artin v-stacks}  Let $f\from X\to Y$ be a proper morphism of $S$-Artin v-stacks over a base $S$.   There exists a natural map 
%\[ f_\natural\from H^0(\In_S(X), K_{\In_S(X)/S}) 
%\to H^0(\In_S(Y), K_{\In_S(Y)/S}). \] 
%If $A\in D_{\et}(X,\Lambda)$ is ULA over $S$, then so is $Rf_*A$, and 
%\[ f_\natural \trdist(A) = \trdist(Rf_* A). \]
%\end{thm}
The Lefschetz-Verdier trace formula was expressed elegantly by Lu and Zheng \cite{LuZheng} in the language of symmetric monoidal 2-categories.  \cite{LuZheng} works with schemes, but our treatment of Artin v-stacks is virtually identical.  First we recall some definitions and constructions concerning the categorical trace.

\begin{dfn}[{\cite[Definition 1.1, Construction 1.6]{LuZheng}}]
An object $X$ of a symmetric monoidal category $(\mc{C},\otimes,1_{\mc{C}})$ is {\em dualizable} if there exists an object $X^\vee$ together with morphisms $\text{ev}_X\from X^\vee\otimes X \to 1_{\mc{C}}$ and $\text{coev}_X\from 1_{\mc{C}} \to X\otimes X^\vee$, such that the compositions

\[
\xymatrix{
X \ar[rr]^{\text{coev}_X\otimes \id_X\hspace{1cm}}
&&
X\otimes X^\vee \otimes X \ar[rr]^{\hspace{1cm}\id_X \otimes \text{ev}_X}
&& X
}
\]
and
\[
\xymatrix{
X^\vee \ar[rr]^{\id_{X^\vee}\otimes\text{coev}_X\hspace{1cm}}
&&
X^\vee \otimes X \otimes X^\vee \ar[rr]^{\hspace{1cm}\text{ev}_X\otimes \id_X}
&& X^\vee
}
\]
are isomorphic to the identities on $X$ and $X^\vee$, respectively.  Equivalently, the functor $Y\mapsto X\otimes Y$ has right adjoint $Y\mapsto X^\vee\otimes Y$.  If $X$ is dualizable, then $X^\vee\otimes Y$ serves as an internal mapping object $\iHom(X,Y)$.   

Let $\Omega\mc{C}=\End(1_{\mc{C}})$ be the (1-)category of endomorphisms of the unit object of $\mc{C}$.  Let $f\in \End X$ be an endomorphism of a dualizable object $X$.  Define the categorical trace $\tr(f)$ as the composite:
\[
\xymatrix{
1_{\mc{C}} \ar[rr]^{\text{coev}_X} &&
X\otimes X^\vee \ar[rr]^{f\otimes \id_{X^\vee}} &&
X\otimes X^\vee \ar[rr]^{\text{ev}_X} &&
1_{\mc{C}}
}
\]
so that $\tr(f)$ is an object of $\Omega\mc{C}$.
\end{dfn}



\begin{dfn}[The category of correspondences] We define a symmetric monoidal 2-category $\Corr_S$. 
The objects of $\Corr_S$ are $S$-Artin v-stacks, which are smooth-locally nice over $S$.  Given objects $X$ and $X'$, the category $\Hom_{\Corr_S}(X,X')$ has for its objects the correspondences:
\begin{equation}
\label{EqCorrespondence}
\xymatrix{
& C \ar[dl]_{c_1} \ar[dr]^{c_2} & \\
X && X'
}
\end{equation}
with each $c_i$ a morphism of $S$-Artin v-stacks, with $c_2$ assumed to be smooth-locally nice.  The composition of $(c_1,c_2)\from C\to X\times_S X'$ with $(d_1,d_2)\from D\to X'\times_S X''$ is the correspondence $(c_1d_1',d_2c_2')$ defined by the diagram:
\begin{equation}
\label{EqCompositionOfCorrespondences}
\xymatrix{
& & C\times_{X'} D \ar[dl]_{d_1'} \ar[dr]^{c_2'} && \\
& C \ar[dl]_{c_1} \ar[dr]^{c_2} && D \ar[dl]_{d_1} \ar[dr]^{d_2}  & \\
X && X' && X'' 
}
\end{equation}
If $c=(c_1,c_2)\from C\to X\times_S X'$ and $c'=(c_1',c_2')\from C'\to X\times_S X'$ represent two objects in $\Hom_{\Corr_S}(X_1,X_2)$, a 2-morphism $c\implies c'$ is a {\em proper} morphism $p\from C\to C'$ such that the following diagram commutes:
\begin{equation}
\label{EqTwoMorphism}
\xymatrix{
& C \ar[dl]_{c_1} \ar[dr]^{c_2} \ar[dd]_p & \\
X & & X' \\
& D \ar[ul]^{c_1'} \ar[ur]_{c_2'} &
}
\end{equation}
The monoidal structure is defined by $X_1\otimes X_2 = X_1\times_S X_2$, with unit object $S$.  Given $c=(c_1,c_2)\from C\to X_1\times_S X'_1$ and $d=(d_1,d_2)\from D\to X_2\times_S X_2'$ representing objects in $\Hom_{\Corr_S}(X_1,X_1')$ and $\Hom_{\Corr_S}(X_2,X_2')$ respectively, we define the object $c\otimes d$ of $\Hom_{\Corr_S}(X_1\times_S X_2,X_1'\times_S X_2')$ as the correspondence: 
\begin{equation}
\label{EqProductCorrespondence}
\xymatrix{
& C\times_S D \ar[dl]_{c_1\times_S d_1} \ar[dr]^{c_2\times_S d_2} &\\
X_1\times_S X_2 && X_1'\times_S X_2'
}
\end{equation}
\end{dfn}


\begin{dfn} [The category of cohomological correspondences] \label{DefCoCorr} We define a symmetric monoidal 2-category $\CoCorr_S$, which comes equipped with a functor to $\Corr_S$.  An object of $\CoCorr_S$ is a pair $(X,A)$, where $X$ is an $S$-Artin v-stack which is smooth-locally nice over $S$, and $A\in D_{\et}(X,\Lambda)$.  Given objects $\mf{X}=(X,A)$ and $\mf{X}'=(X',A')$ of $\CoCorr_S$,  the category $\Hom_{\CoCorr_S}(\mf{X},\mf{X}')$ consists of pairs $(c,u)$, where $c=(c_1,c_2)$ is a correspondence as in \eqref{EqCorrespondence}, and $u\from c_1^*A\to c_2^!A'$ is a morphism in $D_{\et}(C,\Lambda)$.  The composition of $(c,u)\from (X,A)\to (X',A')$ with $(d,v)\from (X',A')\to (X'',A'')$ is $(e,w)$, where $e\from C\times_{X'} D\to X\times_S X''$ is the correspondence in \eqref{EqCompositionOfCorrespondences}, and $w$ is the composition
\[ (d_1')^*c_1^*A\stackrel{u}{\to} (d_1')^*c_2^! A' \stackrel{\alpha}{\to} (c_2')^!d_1^*A' \stackrel{v}{\to} (c_2')^! d_2^! A'' \]
where $\alpha$ is adjoint to the base change isomorphism $(c_2')_!(d_1')^* \isom d_1^* (c_2)_!$.   If $\mf{f}=(c,u)$ and $\mf{f}'=(c',u')$ are two objects in $\Hom_{\CoCorr_S}(\mf{X},\mf{X}')$, a 2-morphism $\mf{f}\implies \mf{f}'$ is a proper morphism $p$ as in \eqref{EqTwoMorphism}, such that $u'$ is the composition 
\begin{eqnarray*}
 (c_1')^*A &\stackrel{\text{unit}}{\to}& p_*p^*(c_1')^*A\isom p_* c_1^*A \stackrel{u}{\to} p_* c_2^! A' \\
 & \isom& p_* p^! (c_2')^! A' \isom p_!p^! (c_2')^! A' \stackrel{\text{counit}}{\to} (c_2')^! A'. 
\end{eqnarray*}
The symmetric monoidal structure on $\Corr_S$ is given by $(X,A)\otimes (X',A')= (X\times_S X', A\boxtimes_S A')$.  The unit object is $1_{\CoCorr_S}=(S,\Lambda_S)$.  Finally, given $(c,u)\from (X_1,A_1)\to (X'_1,A'_1)$ and $(d,v)\from (X_2,A_2)\to (X'_2,A'_2)$, the tensor product $(c,u)\otimes (d,v)$ is $(c\otimes d, w)$, where $c\otimes d$ is the correspondence in \eqref{EqProductCorrespondence}, and $w$ is the composition
\[ (c_1\times_S d_1)^*(A_1\boxtimes_S A_2)\isom c_1^*A_1 \boxtimes d_1^*A_2 \stackrel{u\boxtimes_S v}{\to} c_2^!A_1' \boxtimes_S d_2^!A_2' \stackrel{\kappa}{\to} (c_2\times_S d_2)^! (A_2\boxtimes A_2'), \]
where $\kappa$ is adjoint to the K\"unneth isomorphism $(c_2\times d_2)_!(B_1\boxtimes_S B_2)\isom (c_2)_!B_1 \boxtimes_S (d_2)_!B_2$.  
\end{dfn}

The category $\CoCorr_S$ has internal mapping objects:  if $\mf{X}_1=(X_1,A_1)$ and $\mf{X}_2=(X_2,A_2)$, then $\iHom(\mf{X}_1,\mf{X}_2)=(X_1\times_S X_2,\RHom(\pr_1^*A_1,\pr_2^!A_2))$, where $\pr_i\from X_1\times_S X_2\to X_i$ is the projection.  


%Let $F\from \CoCorr_S\to\Corr_S$ be the forgetful functor.   An important feature of this construction is that if $f\from \mf{X}\to \mf{X}'$ is a morphism, and $F(f)\implies g$ is a 2-morphism, then there exists a unique 

We have the following characterization of dualizable objects in $\CoCorr_S$.

\begin{pro} Let $X$ be an $S$-Artin v-stack, with smooth-locally nice structure map $\pi\from X\to S$, and let $A\in D_{\et}(X,\Lambda)$.  The following are equivalent.
\begin{enumerate}
\item The object $(X,A)$ is dualizable in $\CoCorr_S$.
\item The natural map $m\from \D_{X/S} A\boxtimes_S A \to \RHom(\pr_1^*A,\pr_2^!A)$ (see proof for construction) is an isomorphism.
\end{enumerate}
In this situation, the dual of $(X,A)$ is $(X,\D_{X/S}A)$.
\end{pro} 

\begin{proof} Let $\mf{X}=(X,A)$, and let $\mf{X}'=(X,\D_{X/S}A)$.  There is a morphism $\mf{e}\from \mf{X}'\otimes \mf{X}\to 1_{\CoCorr_S}$, defined as the pair $(c,u)$, where $c=(\Delta_{X/S},\pi)$ and $u$ is the composition 
\[\Delta_{X/S}^*(\D_{X/S} A \boxtimes_S A) \isomto \D_{X/S} A \otimes A \to K_{X/S}=\pi^!\Lambda_S.\]
Then $\mf{e}$ induces a morphism $\mf{X}'\otimes \mf{Y}\to \iHom(\mf{X},\mf{Y})$ for any object $\mf{Y}$ of $\CoCorr_S$.  For $\mf{Y}=\mf{X}$, the map $u$ becomes the map $m$ in (2).

Suppose $\mf{X}$ is dualizable, with witnesses $\mf{X}^\vee$, $\ev_{\mf{X}}$, and $\coev_{\mf{X}}$.   Then $\mf{X}^\vee\otimes \mf{Y}\to \iHom(\mf{X},\mf{Y})$ is an isomorphism for all objects $\mf{Y}$.   Setting $\mf{Y}=1_{\CoCorr_S}$, we find an isomorphism $\mf{X}^\vee\isom \mf{X}'$ which identifies $\ev_{\mf{X}}$ with $\mf{e}$.  Setting $\mf{Y}=\mf{X}$, we find that $m$ is an isomorphism.  

Conversely, if $m$ is an isomorphism, let $\coev_{\mf{X}}=(d,w)$, where $d=(\pi,\Delta_{X/S})$ and $w$ is the composition
\[
\pi^*\Lambda_S \isom \Lambda_X \stackrel{\epsilon}{\to} \RHom_\Lambda(A,A) 
\stackrel{(P5)}{\isomto}  \Delta_{X/S}^!\RHom_\Lambda(\pr_1^*A, \pr_2^!A) 
\]
followed by $m^{-1}\from \Delta_{X/S}^!\RHom_\Lambda(\pr_1^*A, \pr_2^!A)\to \Delta_{X/S}^!(A\boxtimes_S \D_{X/S}A)$.  Here $\epsilon$ is adjont to $\id_A\from A\to A$.  A diagram chase now shows that $\coev_{\mf{X}}$ and $\ev_{\mf{X}}$ witness the dualizability of $\mf{X}$.
\end{proof}  

In the scheme setting, a pair $(X,A)$ is dualizable if and only if $A$ is locally acyclic over $S$ \cite[Theorem 2.16]{LuZheng}, under some mild assumptions.  Similarly, if $X\to S$ is a nice morphism of v-stacks, then $(X,A)$ is dualizable if and only if $A$ is universally locally acyclic over $S$ \cite[Theorem IV.2.24]{FarguesScholze}.  That result extends to the situation of stacky morphisms.  If $X\to S$ is smooth-locally nice,  with uniformization $U\to X$, then $(X,A)$ is dualizable if and only if $A\vert_U$ is ULA over $S$.  

If $\mf{X}$ is a dualizable object of $\CoCorr_S$, and $\mf{f}\from \mf{X}\to \mf{X}$ is an endomorphism, we may define the categorical trace $\tr(\mf{f})$, an object of $\Omega\CoCorr_S=\End 1_{\CoCorr_S}$.  Let us make this explicit.  The category $\Omega\CoCorr_S$ has objects $(X,\omega)$, where $X$ is an $S$-Artin v-stack and $\omega\in H^0(X,K_{X/S})$.  A morphism $(X,\omega)\to (X',\omega')$ is a diagram
\[
\xymatrix{
X\ar[rr]^p \ar[dr]_\pi && X' \ar[dl]^{\pi'} \\
& S & }
\]
with $p$ proper, such that $\omega'=p_*\omega$.  Here \[ p_*\from H^0(X,K_{X/S})\to H^0(X',K_{X'/S}) \]
is induced from $\pi_*K_{X/S}\isom \pi'_*p_*p^!K_{X'/S} \isom \pi'_*p_!p^!K_{X'/S} \stackrel{\text{counit}}{\to} \pi'_*K_{X'/S}$.  

Now let $\mf{X}=(X,A)$ be a dualizable object and let $\mf{f}=(c,u)\from \mf{X}\to \mf{X}$ be an endomorphism, with $c=(c_1,c_2)\from C\to X\times_S X$ and $u\from c_1^*A\to c_2^!A$.  By definition, $\tr(\mf{f}) = \ev_{\mf{X}}\circ (f\otimes \id_{X^\vee}) \circ \coev_{\mf{X}}$.   Let us make explicit $\tr(\mf{f})$.  It is represented by a pair $(\tr(c),\tr(u))$.  Here $\tr(c)\in \Omega 1_{\Corr_S}$ is the correspondence $\Fix(c)\to S\times_S S = S$, where $\Fix(c)$ is the fixed-point locus of the correspondence $c$, as in the cartesian diagram:
\[
\xymatrix{
\Fix(c) \ar[r]^{c'} \ar[d]_{\Delta'_{X/S}} & X \ar[d]^{\Delta_{X/S}} \\
C \ar[r]_c & X\times_S X
}
\]
For its part, the element $\tr(u)$ is an element of $H^0(\Fix(c),K_{\Fix(c)/S})$.   It is the image of $u\in \Hom(c_1^*A,c_2^!A)$ under
\begin{eqnarray*}
H^0(C,\RHom(c_1^*A, c_2^!A)) 
&\stackrel{(P5)}{\isomto}& H^0(C,c^!\RHom(\pr_1^*A, \pr_2^!A)) \\
&\stackrel{\eqref{EqCrucialIsomorphismSchemes}}{\isomto}& H^0(C,c^!(\D_{X/S}A \boxtimes_S A)) \\
&\stackrel{\alpha}{\to}& H^0(C,c^!(\Delta_{X/S})_* (\D_{X/S}A \otimes A) ) \\
&\stackrel{\ev_A}{\to}& H^0(C,c^!(\Delta_{X/S})_* K_{X/S} )\\
&\stackrel{{\text{(BC2)}}}{\isomto}& H^0(C,(\Delta'_{X/S})_* (c')^! K_{X/S}) \\
&\isom&  H^0(\Fix(c),K_{\Fix(c)/S}).
\end{eqnarray*}
Here, the map labeled $\alpha$ is adjoint to $(\Delta_{X/S})^*(\D_{X/S}A \boxtimes_S A)\isomto \D_{X/S} A \otimes A$.   

\begin{dfn}[Inertia stack, characteristic class]
In the special case that $\mf{f}=\id_{\mf{X}}=(\Delta_{X/S},\id_A)$, the object $\tr(\Delta_{X/S})=X\times_{X\times_S X} X$ is the {\em inertia stack} of $X$, which we notate as $\In_S(X)$.  Its objects are pairs $(x,g)$, where $x\in X$ and $g\in \Aut x$.  Then $\tr(\id_A)$ is an element of $H^0(\In_S(X),K_{\In_S(X)})$, which we call the {\em characteristic class} of $\mf{X}$.   We notate this as $\cc_{X/S}(A)$. 
\end{dfn}

We record one lemma here for later reference.

\begin{lem}\label{LemRestrictionOfCC} Let $i\from U\to X$ be an open immersion of $S$-Artin v-stacks.  Then $\In_S(i)\from \In_S(U)\to \In_S(X)$ is also an open immersion.  If $A\in D_{\et}(X,\Lambda)$ is ULA over $S$, then so is $i^*A$, and then 
\[ \cc_{U/S}(i^*A)=\In_S(i)^*\cc_{X/S}(A). \]
\end{lem}

\begin{proof} All constructions are local on $X$.
\end{proof}



\begin{thm}[Relative Lefschetz-Verdier trace formula]  \label{ThmLefschetzVerdier} Let $\mf{X}=(X,A)$ be a dualizable object, and let $\mf{f}\in \End \mf{X}$ lie over the correspondence $c\from C\to X\times_S X$.  Suppose we are given a diagram
\[ 
\xymatrix{
X \ar[d]_{q} & C\ar[l] \ar[r] \ar[d]_p & X \ar[d]_{q} \\
X' & C'\ar[l] \ar[r] & X' 
}
\]
with $p,q$ proper.  Then $\mf{X}'=(X',q_*A)$ is also dualizable.   Let $\mf{q}\from \mf{X}\to \mf{X}'$ be the evident 1-morphism lying over $q$.  There is a unique morphism $\mf{f}'\in \End\mf{X}'$ lying over $C'\to X'\times_S X'$, such that $p$ defines a 2-morphism $\tilde{p}$ filling in the square
\[
\xymatrix{
 \mf{X} \ar[r]^{\mf{f}} \ar[d]_{\mf{q}} & \mf{X} \ar[d]^{\mf{q}} \\
\mf{X}' \ar[r]_{\mf{f}'} & \mf{X}'
} 
\]
Finally, there exists a (necessarily unique) 2-morphism $\tr(\tilde{p})\from \tr(\mf{f})\implies \tr(\mf{f}')$ lying over $\tr(p)\from \tr(c)\implies \tr(c')$.  
\end{thm}

\begin{proof}  This is formally the same as the proof of \cite[Theorem]{LuZheng}, so we give a brief sketch.  (In \cite{LuZheng} one gets a statement about the more general Lefschetz-Verdier pairing, which we also could have established.)   The existence and uniqueness of $\mf{f}'\in \End\mf{X}'$ follows from the definition of 2-morphisms in $\CoCorr_S$.   The dualizability of $\mf{X}'$ is \cite[Proposition 2.23]{LuZheng}.  
The dual of $\mf{X}'$ is $(\mf{X}')^\vee=(X',q_*\D_{X/S}A)$;  there is another natural map $\mf{q}^\vee\from \mf{X}^\vee\to (\mf{X}')^\vee$ defined similarly to $\mf{q}$.  

Consider the diagram:
\[
\xymatrix{
1_{\CoCorr_S} \ar[r]^{\coev_{\mf{X}}} \ar[dr]_{\coev_{\mf{X}'}} & \mf{X}\otimes \mf{X}^\vee \ar[d]^{\mf{q}\otimes \mf{q}^\vee} \ar[r]^{\mf{f}\otimes\id_{\mf{X}^\vee}} & \mf{X} \otimes \mf{X}^\vee \ar[d]_{\mf{q}\otimes \mf{q}^\vee} \ar[dr]^{\ev_{\mf{X}}} & \\
& \mf{X}'\otimes (\mf{X}')^\vee \ar[r]_{\mf{f}'\otimes\id_{\mf{X}'}} & \mf{X}'\otimes (\mf{X}')^{\vee} \ar[r]_{\ev_{\mf{X}'}} & 1_{\CoCorr_S} 
}
\]
The two outer triangles can be filled in with a 2-morphism, as can the inner square (via $p\otimes\id_{\mf{q}^{\vee}}$).  See \cite[Construction 1.7]{LuZheng} for details.  Composing, we find the required 2-morphism $\tr(\tilde{p})\from \tr(\mf{f})\implies \tr(\mf{f}')$.  
\end{proof}

\begin{cor}\label{CorLefschetzVerdier} Let $(X,A)$ be a dualizable object, and let $p\from X\to X'$ be proper.  Then $(X',p_!A)$ is dualizable.  The morphism $\In_S(p)\from \In_S(X)\to \In_S(X')$ is proper, and 
\[ \In_S(p)_*\cc_{X/S}(A) = \cc_{X'/S}(p_!A).\]
\end{cor}

We can immediately deduce a familiar-looking trace formula from Theorem \ref{ThmLefschetzVerdier} in the case of proper diamonds.   Suppose $S=\Spd C$ for an algebraically closed perfectoid field $C$, and suppose $q\from X\to S$ is a nice diamond.  Let $A\in D_{\et}(X,\Lambda)$ be ULA over $S$.  Then $\mf{X}=(X,A)$ is a dualizable object of $\CoCorr_S$.   Let $\mf{f}=(c,u)$ be an endomorphism of $\mf{X}$ lying over a correspondence $c\from Y\to X\times_S X$.  The categorical trace $\tr(\mf{f})$ is an endomorphism of $1_{\CoCorr_S}$ consisting of the pair $(\Fix(c),\omega)$, where $\Fix(c)=Y\times_{c,X\times_S X,\Delta_{X/S}} X$ is the fixed point locus of the correspondence, and $\omega$ is a global section of $K_{\Fix(c)/S}$.  

Now suppose that $X$ and $Y$ are both proper over $S$.  In the setting of Theorem \ref{ThmLefschetzVerdier}, we put $\mf{X}'=(S,q_*A)$ and $C'=S$.   The dualizability of $\mf{X}'$ means that $q_*A=R\Gamma(X,A)$ is a perfect complex.  The morphism $\mf{f}'\from \mf{X}'\to \mf{X}'$ supplied by Theorem \ref{ThmLefschetzVerdier} is the endomorphism $q_*(\mf{f})\from q_*A \to q_*A$.  Finally, the existence of $\tr(\tilde{p})\from \tr(\mf{f})\implies \tr(\mf{f}')$ lying over $\tr(p)\from \tr(c)\implies \tr(\id_S)$ implies that 
\begin{equation}
\label{EqLefschetzProperDiamonds}
\tr\left(q_*(\mf{f})\biggm\vert R\Gamma(X,A)\right) = \int_{\Fix(c)} \omega.
\end{equation}

\begin{dfn} Let $x\in \Fix(c)$ be an isolated point, such that $x\to S$ an isomorphism.   The {\em local term} $\loc_x(\mf{f})$ is the restriction of $\omega$ to $x$, considered as an element of $\Lambda$.  

If $\mf{f}$ arises from an automorphism $g\from X\to X$ along with a morphism $u\from g^*A\to A$, we write the local term as $\loc_x(g,A)$ (the dependence on $u$ being implicit).
\end{dfn}

In the latter situation, if it so happens that $\Fix(g)$ consists of finitely many isolated $S$-points $x_1,\dots,x_n$, then \eqref{EqLefschetzProperDiamonds} reduces to
\[ \tr\left(q_*(g)\biggm\vert R\Gamma(X,A)\right) = \sum_{i=1}^n \loc_x(g,A).\]



\subsection{Examples}

In the following, assume $S=\Spd C$ for an algebraically closed perfectoid field $C$, or else $S=\Spd k$ for an algebraically closed discrete field of characteristic $p$.   In both cases, we freely identify $D_{\et}(S,\Lambda)$ with the derived category of $\Lambda$-modules.

\begin{exm} An object $A\in D_{\et}(S,\Lambda)$ is ULA over $S$ if and only if (when considered as a complex of $\Lambda$-modules) $A$ is perfect.  (See Lemma \ref{lem:reflexivemodules} in the Appendix for a proof of this claim and related conditions.)
\end{exm}

\begin{exm} Let $T$ be a locally profinite set, and let $T_S=\underline{T} \times S$ be the associated constant diamond over $S$.  Then $f\from T_S\to S$ is nice. Let $C(T,\Lambda)$ be the ring of continuous functions $T\to \Lambda$, for the discrete topology on $\Lambda$.  We may naturally identify $D_{\et}(T_S,\Lambda)$ with the derived category of the abelian category of smooth $C(T,\Lambda)$-modules in the sense of \S \ref{Sheaveslpfsets}. Indeed, $D_{\et}(T_S,\Lambda) \cong D(T_{S,\et},\Lambda)$ since $T_S$ locally has cohomological dimension zero, so it is enough to identify $\mathrm{Sh}(T_{S,\et},\Lambda)$ with the category of smooth $C(T,\Lambda)$-modules, which is Lemma \ref{lem:sheaflps}. This identification matches the constant sheaf $\Lambda$ with the smooth $C(T,\Lambda)$-module $C_c(T,\Lambda)$. Under this identification, we have concrete descriptions of the four operations associated with $f$ (where we freely use some language and notation from \S \ref{Sheaveslpfsets}):
\begin{itemize}
\item $f^*$ sends a $\Lambda$-module $M$ to the smooth $C(T,\Lambda)$-module $C_c(T,\Lambda)\otimes_\Lambda M$,
\item $f_*$ sends a smooth $C(T,\Lambda)$-module $M$ to $M^c$ regarded as a $\Lambda$-module.
\item $f_!$ sends a smooth $C(T,\Lambda)$-module $M$ to its underlying $\Lambda$-module.
\item $f^!$ sends a $\Lambda$-module $M$ to $\Rhom_\Lambda(C_c(T,\Lambda),M)^s$.  In particular $H^0(T_S, f^!\Lambda_S) \isom \Dist(T,\Lambda)$, the module of $\Lambda$-valued distributions on $T$.
\end{itemize}
It will not generally be true that $\Lambda_{T_S}$ is ULA over $S$, unless $T$ is discrete.
\end{exm}

\begin{exm} \label{ExLocallyProPGroup} Suppose $G$ is a locally pro-$p$ group.  Let $[S/G_S]$ be the classifying v-stack of $G_S$-torsors.  We assume that there is a free action of $G_S$ on a cohomologically smooth diamond $X\to S$.   In that case $[S/G_S]$ has a cohomologically smooth uniformization by the cohomologically smooth diamond $X/G_S$;  thus $[S/G_S]$ is a smooth $S$-Artin v-stack.  Then $K_{[S/G]/S}$ is the invertible sheaf associated with the module $\mathrm{Haar}(G,\Lambda)$ of $\Lambda$-valued Haar measures on $G$.

We may identify $D_{\et}([S/G_S],\Lambda)$ with the derived category of $\Lambda$-modules with a smooth $G$-action \cite[Theorem V.1.1]{FarguesScholze}.  If $\pi$ is a smooth representation of $G$ on a $\Lambda$-module, let $[\pi]$ denote the corresponding object of $D_{\et}([S/G_S],\Lambda)$.  The object $[\pi]$ is ULA over $S$ if and only if $\pi$ is admissible, by which we mean the condition that the derived $K$-invariants of $\pi$ are a perfect complex for all compact open $K\subset G$.  In that case, $\D_{[S/G_S]/S}[\pi]\isom [\pi^\vee] \otimes K_{[S/G]/S}$
is the smooth dual twisted by the module of Haar measures.
\end{exm}

\begin{exm} Let $G$ be a locally pro-$p$ group as in Example \ref{ExLocallyProPGroup}.   Let $T$ be a locally profinite set equipped with a continuous action of $G$, and let $T_S$ be the constant diamond over $S$.  The stacky quotient $[T_S/G_S]$ is an $S$-Artin v-stack;  it is uniformized by $(X\times_S T_S)/G_S$.  It is not in general cohomologically smooth over $S$.  The category $D_{\et}([T_S/G_S],\Lambda)$ may be identified with the derived category of $G$-equivariant smooth $C(T,\Lambda)$-modules. Using this identification, we get a natural isomorphism $H^0([T_S / G_S],K_{[T_S/G_S]/S}) \isom \Dist(T,\mathrm{Haar}(G,\Lambda))^G$, the module of $G$-invariant distributions on $T$ with values in $\mathrm{Haar}(G,\Lambda)$.  If $G$ is unimodular, and if we choose a Haar measure on $G$, then this is isomorphic to $\Dist(T,\Lambda)^G$.  

A stack of this form appears as the inertia stack of $[S/G_S]$.  Indeed, $\In_S([S/G_S])\isom [G_S\sslash G_S]$ is the stack of conjugacy classes of $G$.  (Reasoning:  For a perfectoid space $Y\to S$, a $Y$-point of $\In_S([S/G_S])$ is a $G_S$-torsor $\tilde{Y}\to Y$ together with a $G_S$-equivariant automorphism $i\from \tilde{Y}\to \tilde{Y}$.  Such an automorphism arises as $i(y)=f(y).y$, where $f\from \tilde{Y}\to G_S$ is a morphism satisfying $f(gy)=gf(y)g^{-1}$.  The pair $(\tilde{Y},f)$ then constitutes a $Y$-point of $[G_S\sslash G_S]$.)

Suppose now that $G$ is unimodular, and suppose we have chosen a Haar measure on it.   Let $\pi$ be a smooth admissible representation of $G$ on a $\Lambda$-module.  Then $\cc_{[S/G_S]/S}([\pi])$ is an element of 
\[ H^0([G_S\sslash G_S], K_{[G_S\sslash G_S]/S}) \isom \Dist(G,\Lambda)^G, \]
the module of conjugacy-invariant $\Lambda$-valued distributions on $G$.  This element is none other than the trace distribution of $\pi$.  
\end{exm}


\subsection{A K\"unneth theorem for characteristic classes}

The goal of this section is to prove the compatibility of the categorical trace with fiber products, to get an analogue of the relation $\tr(A\otimes B)=\tr(A) \tr(B)$ for square matrices.  

As an example of what we will do, suppose $X_1,X_2\to S$ are two smooth-locally nice morphisms of $S$-Artin v-stacks, and suppose $A_i\in D_{\et}(X_i,\Lambda)$ is ULA over $S$ for $i=1,2$.  Then $A_1\boxtimes_S A_2$ is ULA over $S$, so we may define the characteristic class $\cc_{X_1\times_S X_2/S}(A_1\boxtimes_S A_2)$ in $H^0(\In_S(X_1\times_S X_2),K_{\In_S(X_1\times_S X_2)})$.  We have an isomorphism $\In_S(X_1\times_S X_2)\isom \In_S(X_1)\times_S \In_S(X_2)$, and therefore a K\"unneth map 
\begin{eqnarray*}
\kappa_S \from K_{\In_S(X_1)/S} \otimes K_{\In_S(X_2)/S} \to K_{\In_S(X_1\times_S X_2)/S}
\end{eqnarray*}
which we notate as $\mu_1\otimes\mu_2\mapsto \mu_1\boxtimes_S \mu_2$ for global sections $\mu_i$ of $K_{\In_S(X_i)/S}$.  Then it is straightforward to show (and a corollary of Theorem \ref{ThmKunnethForCharacteristicClass} below) that 
\[ \cc_{X_1/S}(A_1)\boxtimes_S \cc_{X_2/S}(A_2)=\cc_{X_1\times_S X_2/S}(A_1\boxtimes_S A_2).\]

For our applications we need a more general result involving fiber products over bases other than $S$.  First, we need a modification of the above K\"unneth map in a general setting.

\begin{dfn}[Modified K\"unneth map]  Let $U\to T$ be a cohomologically smooth morphism of $S$-Artin v-stacks. Suppose we are given a commutative diagram of $S$-Artin v-stacks
\[ 
\xymatrix{
Y_i \ar[r]^{f_i} \ar[d]_{g_i} & X_i \ar[d] \\
U \ar[r] & T
}
\]
for $i=1,2$.   Let $f\from Y_1\times_U Y_2\to X_1\times_T X_2$ and $g\from Y_1\times_U Y_2 \to U$ be the induced product maps.  Let $A_i$ be an object of $D_{\et}(X_i,\Lambda)$ for $i=1,2$.  We define a map
\[ \kappa_{U/T}\from f_1^!A_1 \boxtimes_U f_2^!A_2 \to f^!(A_1\boxtimes_T A_2) \otimes g^*K_{U/T} \]
as follows.  There is a cartesian diagram
\[
\xymatrix{
Y_1\times_U Y_2 \ar[r]^{\Delta_{U/T}'} \ar[d]_g & Y_1\times_T Y_2 \ar[d]^{g_1\times_T g_2} \\
U \ar[r]_{\Delta_{U/T}} & U\times_T U 
}
\]
The map $\kappa_{U/T}$ is defined as the composition
\begin{eqnarray*}
&&f_1^!A_1\boxtimes_U f_2^!A_2 \\
&\isom& (\Delta_{U/T}')^*(f_1^!A_1 \boxtimes_T f_2^!A_2) \\
&\to& (\Delta_{U/T}')^*(f_1\times_T f_2)^!(A_1\boxtimes_T A_2) \\
&\stackrel{\eqref{EqInverseDualizingComplexes}}{\isom}& (\Delta_{U/T}')^*(f_1\times_T f_2)^!(A_1\boxtimes_T A_2) \otimes g^*(\Delta_{U/T})^!\Lambda_T \otimes g^*K_{U/T} \\
&\to& (\Delta_{U/T}')^*(f_1\times_T f_2)^! (A_1\boxtimes_T A_2) \otimes (\Delta_{U/T}')^!\Lambda_{Y_1\times_T Y_2} \otimes g^*K_{U/T} \\
&\to& (\Delta_{U/T}')^!(f_1\times_T f_2)^!(A_1\boxtimes_T A_2) \otimes g^*K_{U/T} \\
&\isom& f^!(A_1\boxtimes_T A_2) \otimes g^*K_{U/T}.
\end{eqnarray*}
\end{dfn}

In particular the case $X_1=X_2=T=S$ yields a map 
\begin{equation}
\label{EqModifiedKunneth}
 \kappa_{U/S} \from K_{Y_1/S} \boxtimes_U K_{Y_2/S} \to K_{Y_1\times_U Y_2/S} \otimes g^*K_{U/S}.
 \end{equation}

We can now introduce the setup of the main theorem of this section.  We consider bases $T\to S$ satisfying two hypotheses:  (1) $T\to S$ is cohomologically smooth, and (2) $\Delta_{T/S}\from T\to T\times_S T$ is cohomologically smooth.  These are satisfied for instance when $T=[S/G]$, where $G$ is a cohomologically smooth group diamond over $S$.  Considering the diagram
\[
\xymatrix{
\In_S(T) \ar[r] \ar[d] & T \ar[d]^{\Delta_{T/S}} & \\
T \ar[r]_{\Delta_{T/S}} & T\times_S T\ar[r] \ar[d] & T \ar[d] \\
& T \ar[r] & S
}
\]
in which both squares are cartesian, we see that $\In_S(T)\to S$ is also cohomologically smooth.   Furthermore we can trivialize the dualizing complex $K_{\In_S(T)/S}$.

\begin{lem}  \label{LemTrivialDualizingSheaf} Let $T$ be an $S$-Artin v-stack such that the structure map $\pi\from T\to S$ and diagonal $\Delta_{T/S} \from T\to T\times_S T$ are both cohomologically smooth.   Then the object $\mf{T}=(T,\Lambda_T)\in\CoCorr_S$ is dualizable, and its characteristic class $\cc_{T/S}(\Lambda_T)$, considered as a morphism $\Lambda_{\In_S(T)} \to K_{\In_S(T)/S}$, is an isomorphism.
\end{lem}

In the case $T=[S/G]$, where $G$ is a cohomologically smooth group diamond over $S$, the inertia stack is $\In_S(T)=[G\sslash G]$, the stack of conjugacy classes of $G$.  This is a cohomologically smooth stack of dimension 0, so perhaps it is unsurprising that it has trivial dualizing complex;  the lemma states that the trivialization is in fact canonical.

\begin{proof} Let $\pr_1,\pr_2\from T\times_S T\to T$ be the projection morphisms. The morphism in $D_{\et}(T,\Lambda)$ associated with the cohomological correspondence $\coev_{\mf{T}}\from$ $(S,\Lambda_S)\to (T\times_S T, \pr_2^*K_{T/S})$ is an isomorphism:
\[\pi^*\Lambda_S\isom\Delta_{T/S}^!\pr_1^!\pi^*\Lambda_S \stackrel{\alpha}{\isom} \Delta_{T/S}^!\pr_2^*\pi^!\Lambda_S =  \Delta_{T/S}^!\pr_2^*K_{T/S}. \]
Here we the use cohomological smoothness of $\pi$ to get the isomorphism $\alpha$, as in Theorem \ref{ThmSmoothBaseChange}.   The morphism $\Delta_{T/S}^*\pr_2^*K_{T/S}\to \pi^!\Lambda_S$ associated with $\ev_{\mf{T}}\from (T\times_S T,\pr_2^*K_{T/S})\to (S,\Lambda_S)$ is also an isomorphism (this is true without any hypotheses on $\pi$ or $\Delta_{T/S}$).   Referring to the diagram
\[
\xymatrix{
& & \In_S(T) \ar[dl]_{h} \ar[dr]^{h} && \\
& T \ar[dl]_{\pi} \ar[dr]^{\Delta_{T/S}} && T \ar[dl]_{\Delta_{T/S}} \ar[dr]^{\pi}  & \\
S && T\times_S T && S
}
\]
we may describe the characteristic class $\cc_{T/S}(\Lambda_T)$ as the composition
\begin{eqnarray*}
h^*\pi^*\Lambda_S &\isom&  h^*\Delta_{T/S}^!\pr_2^*K_{T/S}\\&\stackrel{\beta}{\isom}& h^!\Delta_{T/S}^*\pr_2^* K_{T/S}\isom h^!K_{T/S}\isom K_{\In_S(T)/S},
\end{eqnarray*}
which is an isomorphism.  Here we once again applied Theorem \ref{ThmSmoothBaseChange}, using the cohomological smoothness of $\Delta_{T/S}$. 
\end{proof}

Now suppose $p_i\from X_i\to T$ ($i=1,2$) is a morphism of $S$-Artin v-stacks, with fiber product $p\from X_1\times_T X_2\to T$.  There is an isomorphism
\[ \In_S(X_1\times_T X_2) \isom \In_S(X_1)\times_{\In_S(T)} \In_S(X_2), \]
and therefore a modified K\"unneth map 
\[ \kappa_{\In_S(T)/S}\from K_{\In_S(X_1)/S} \boxtimes_{\In_S(T)} K_{\In_S(X_2)/S} \to K_{\In_S(X_1\times_T X_2)/S} \otimes \In(p)^*K_{\In_S(T)/S}. \]
Using the trivialization $\Lambda_{\In_S(T)/S}\isom K_{\In_S(T)/S}$ from Lemma \ref{LemTrivialDualizingSheaf}, we obtain a map
\begin{equation}
\label{EqBoxtimesOnDistributions}
K_{\In_S(X_1)/S} \boxtimes_{\In_S(T)} K_{\In_S(X_2)/S} \to K_{\In_S(X_1\times_T X_2)/S}, 
\end{equation}
which on global sections we notate as $\mu_1\otimes\mu_2\mapsto \mu_1\boxtimes_{\In_S(T)} \mu_2$.  

Finally we can state the main theorem of the section.

\begin{thm} \label{ThmKunnethForCharacteristicClass}  Let $X_1,X_2\to T$ be two morphisms of $S$-Artin v-stacks, and let $A_i\in D_{\et}(X_i,\Lambda)$ be ULA over $S$.  Assume that the structure map $\pi\from T\to S$ and the diagonal $\Delta_{T/S}\from T\to T\times_S T$ are both cohomologically smooth.  Then $A_1\boxtimes_T A_2$ is ULA over $S$, and
\[ \cc_{X_1/S}(A_1)\boxtimes_{\In_S(T)} \cc_{X_2/S}(A_2)
= \cc_{X_1\boxtimes_T X_2/S}(A_1\boxtimes_T A_2). \]
\end{thm}

In order to prove Theorem \ref{ThmKunnethForCharacteristicClass}, we need to enhance the category $\CoCorr_S$ to include data coming from a smooth base v-stack, which we allow to vary.   Such a category would have objects $(X\to T,A)$, where $T\to S$ is cohomologically smooth, $X\to T$ is a morphism of v-stacks, and $A\in D_{\et}(X,\Lambda)$.  The morphisms $(X\to T,A)\to (X'\to T',A')$ would be pairs $(q^\natural,\alpha)$, where $q^\natural =(p,q,p')$ is a morphism of correspondences:
\begin{equation}
\label{EqBasedCorrespondence}
\xymatrix{
X \ar[d]_{p} & C\ar[l]_{c} \ar[d]_{q} \ar[r]^{c} & X' \ar[d]^{p'}\\
T & U \ar[l]_{u} \ar[r]^{u'} & T'
}
\end{equation} 
and $\alpha\from c^*A\to (c')^!A'$ is a morphism.  We assume that $u'$ is cohomologically smooth.

Given pairs $\mf{X}_1=(X_1\to T,A_1)$ and $\mf{X}_2=(X_2\to T,A_2)$ with common base $T$, we could then define $\mf{X}_1\boxtimes_T \mf{X}_2 = (X_1\times_T X_2\to T,A_1\boxtimes_T A_2)$.  However, it turns out that this definition is not functorial in $\mf{X}_1$ and $\mf{X}_2$.  That is: given a morphism $e\from T\to T'$ in $\Corr_S$ and morphisms $f_i\from \mf{X}_i\to \mf{X}_i'$ lying over $e$, one cannot in general define a map $f_1\otimes_e f_2\from \mf{X}_1\boxtimes_T \mf{X}_2\to \mf{X}_1'\boxtimes_{T'} \mf{X}_2'$.  Essentially, this is due to the appearance of the invertible sheaf $K_{U/S}$ appearing in the modified K\"unneth map \eqref{EqModifiedKunneth}.  

To obtain a functorial definition of $\mf{X}_1\boxtimes_T \mf{X}_2$, we need to define an enhancement of the category which keeps track of an invertible sheaf living on the base.

\begin{dfn}[The category of based cohomological correspondences] \label{DefBCoCorr} 
We define a symmetric monoidal 2-category $\BCoCorr_S$.  The objects of $\BCoCorr_S$ are triples $(X\to T,A,B)$, where $X\to T$ is a morphism of $S$-Artin v-stacks,  both smooth-locally nice over $S$, where $A$ is an object of $D_{\et}(X,\Lambda)$, and where $B$ is an {\em invertible} object of $D_{\et}(T,\Lambda)$.   We assume that the structure map $T\to S$ be cohomologically smooth.  Given objects $\mf{X}=(X\to T,A,B)$ and $\mf{X}'=(X'\to T',A',B')$, an object of the category $\Hom_{\BCoCorr_S}(\mf{X},\mf{X}')$ is a triple $(q^\natural,\alpha,\beta)$.  The first element in the triple is a morphism $q^\natural=(p,q,p')$ between correspondences as in \eqref{EqBasedCorrespondence}, where $u'$ is cohomologically smooth.   The second element is a morphism
$\alpha\from c^*A \to (c')^!A'$, and the third is an {\em isomorphism} $\beta\from u^*B\isomto (u')^*B'$.  Compositions of morphisms are defined similarly as in Definition \ref{DefCoCorr}.  (Note that the cohomological smoothness of $u'$ is preserved under composition of correspondences.)  Given objects $(X\to T,A,B)$ and $(X'\to T',B')$, and morphisms between them represented by $C\to X\times_U X'$ (lying over $U\to T\times_S T'$) and $D\to X\times_V X'$ (lying over $V\to T\times_S T'$), a 2-morphism is a pair of proper morphisms $C\to D$ and $U\to V$ making the relevant diagrams commute.   

The monoidal structure on $\BCoCorr_S$ is defined by 
\[ (X\to T,A,B)\otimes (X'\to T',A',B')=(X\times_S X'\to T\times_S T',A\boxtimes_S A',B\boxtimes_S B'). \]
The unit object is $(S,S,\Lambda_S)$.   

Finally, we introduce the obvious monoidal functors $\mc{B},\mc{S}\from \BCoCorr_S\to \CoCorr_S$, with $\mc{B}(X\to T,A,B)=(T,B)$ (the {\em base}) and $\mc{S}(X\to T,A,B)=(X,A)$ (the {\em source}).
\end{dfn}






So far the objects $A$ and $B$ in Definition \ref{DefBCoCorr} have nothing to do with each other.  They only begin to interact when we talk about fiber products of objects of $\BCoCorr_S$ over common bases.   Given objects $\mf{X}_i=(X_i\stackrel{p_i}{\to} T,A_i,B)$ for $i=1,2$ with common base $\mf{T}=(T,B)$, we define
\[ \mf{X}_1\boxtimes_{\mf{T}} \mf{X}_2 = (X_1\times_T X_2\stackrel{p}{\to} T, (A_1\boxtimes_T A_2)\otimes p^*B^{-1}). \]  
We claim that $\boxtimes_{\mf{T}}$ defines a monoidal functor 
\begin{equation}
\label{EqFiberProductFunctor}
\BCoCorr_S \times_{\mc{B},\CoCorr_S} \BCoCorr_S \to \BCoCorr_S.
\end{equation}
A morphism in the category $\BCoCorr_S \times_{\mc{B},\CoCorr_S} \BCoCorr_S$ is a morphism $e\from \mf{T}\to \mf{T}'$ in $\CoCorr_S$ together with a pair of morphisms $\mf{f}_i\from \mf{X}_i\to \mf{X}_i'$ ($i=1,2$) lying over $e$.  We may represent this state of affairs with a diagram 
\begin{equation}
\label{EqMorphismOfCorrespondences}
\xymatrix{
X_i \ar[d]_{p_i} & C_i \ar[l]_{c_i} \ar[d]_{q_i} \ar[r]^{c_i'} & X'_i \ar[d]^{p'_i} \\
T & U \ar[l]_{u} \ar[r]^{u'} & T'
}
\end{equation}
for $i=1,2$, with $u'$ smooth, together with morphisms $\alpha_i\from c_i^*A_i\to (c_i')^!A_i'$ for $i=1,2$ and an isomorphism $\beta\from u^*B\isomto (u')^*B'$.   Taking fiber products over the base correspondence, we obtain a morphism of correspondences $q^\natural=(p,q,p')$ fitting into a diagram 
\begin{equation}
\xymatrix{
X_1\times_T X_2 \ar[d]_{p} & C_1\times_U C_2\ar[d]_{q} \ar[l]_c \ar[r]^{c'} & X_1' \times_{T'} X_2' \ar[d]^{p'} \\
T & U \ar[l]^u \ar[r]_{u'} & T' 
}
\end{equation}
The required morphism
\begin{equation}
\label{EqFiberProductOfCorrespondences}
c^*\left((A_1\boxtimes_T A_2)\otimes p^*B^{-1}\right) \to (c')^!\left((A_1'\boxtimes_{T'} A_2') \otimes (p')^*(B')^{-1}\right)
\end{equation}
is defined as the composition
\begin{eqnarray*}
c^*\left((A_1\boxtimes_T A_2)\otimes p^*B^{-1}\right) &\isom&
(c_1^*A_1 \boxtimes_U c_2^* A_2)\otimes q^*u^*B^{-1} \\
&\stackrel{(\alpha_1\boxtimes_U\alpha_2)\otimes \beta}{\to}&
(c_1')^!A_1' \boxtimes_U (c_2')^!A_2' \otimes q^*((u')^!B')^{-1} \\
&\stackrel{\kappa_{U/T'}}{\to}&
(c')^!(A_1' \boxtimes_{T'} A_2') \otimes q^*(K_{U/T'}\otimes ((u')^!B')^{-1}) \\
&\isom& (c')^!(A_1' \boxtimes_{T'} A_2') \otimes q^*(u')^*(B')^{-1} \\
&\isom& (c')^!\left((A_1'\boxtimes_{T'} A_2') \otimes (p')^*(B')^{-1}\right),
\end{eqnarray*}
where in the last step we used Lemma \ref{LemInvertibleSheaf}.  

To completely justify that \eqref{EqFiberProductFunctor} is a functor, one must also produce a 2-isomorphism
\begin{equation}
\label{EqBoxtimesIsFunctorial}
(\mf{f}_1'\boxtimes_{e'} \mf{f}_2') \circ (\mf{f}_1\boxtimes_e \mf{f}_2) \isom (\mf{f}_1'\circ \mf{f}_1)\boxtimes_{e'\circ e} (\mf{f}_2'\circ \mf{f}_2) 
\end{equation}
whenever all compositions are defined.  Furthermore one must also show that \eqref{EqFiberProductFunctor} is a monoidal functor; that is, we have an isomorphism
\begin{equation}
\label{EqBoxtimesIsTensorFunctor}
 (\mf{X}_1 \boxtimes_{\mf{T}} \mf{X}_2) \otimes (\mf{X}_1'\boxtimes_{\mf{T}'} \mf{X}_2')
\isom (\mf{X}_1\otimes \mf{X}_1')\boxtimes_{\mf{T}\otimes \mf{T}'} (\mf{X}_2\otimes\mf{X}_2'). 
\end{equation}
The details are straightforward but tedious.

We can now prove Theorem \ref{ThmKunnethForCharacteristicClass}.   Let $X_1,X_2\to T$ be two morphisms of $S$-Artin v-stacks, and let $A_i\in D_{\et}(X_i,\Lambda)$ be ULA over $S$.  Assume that the structure map $\pi\from T\to S$ and the diagonal $\Delta_{T/S}$ are both cohomologically smooth. 

Let $\mf{X}_i=(X_i\to T, A_i,\Lambda_T)\in \BCoCorr_S$ for $i=1,2$, so that $\mc{B}(\mf{X}_1)=\mc{B}(\mf{X}_2)=\mf{T}=(T,\Lambda_T)$.  Then $\mf{X}_i$ is dualizable, with dual $\mf{X}_i^\vee=(X_i\to T,\D_{X_i/S}A_i,K_{T/S})$, as witnessed by $\coev_{\mf{X}_i}\from 1_{\BCoCorr_S}\to \mf{X}_i\otimes \mf{X}_i^\vee$ and $\ev_{\mf{X}_i}\from \mf{X}_i^\vee \otimes\mf{X}_i \to 1_{\BCoCorr_S}$.   Note that $\mc{B}(\coev_{\mf{X}_i})=\coev_{\mf{T}}$ and $\mc{S}(\coev_{\mf{X}_i})=\coev_{\mc{S}(\mf{X}_i)}$, and similarly for $\ev$.   Then the categorical trace of $1_{\mf{X}_i}$ is $\tr(1_{\mf{X}_i})=\ev_{\mf{X}_i}\circ \coev_{\mf{X}_i}$, so that $\mc{S}(\tr(1_{\mf{X}_i}))=\tr(1_{\mc{S}(\mf{X}_i)})=\cc_{X_i/S}(A_i)$. 

Now consider $\mf{X}=\mf{X}_1\boxtimes_{\mf{T}} \mf{X}_2=(X_1\boxtimes_T X_2\to T, A_1\boxtimes_T A_2,\Lambda_T)$.  Define an object $\mf{X}^\vee = \mf{X}_1^\vee\boxtimes_{\mf{T}^\vee} \mf{X}_2^\vee$, and define morphisms $\coev_{\mf{X}}$ and $\ev_{\mf{X}}$ via the diagrams
\[
\xymatrix{
1_{\BCoCorr_S} \ar[rrrr]^{\coev_{\mf{X}_1}\boxtimes_{\coev_{\mf{T}}}\coev_{\mf{X}_2}\;\;\;\;} 
 \ar[drrrr]_{\coev_{\mf{X}}} &&&& (\mf{X}_1\otimes\mf{X}_1^\vee)\boxtimes_{\mf{T}\otimes\mf{T}^\vee} (\mf{X}_2\otimes\mf{X}_2^\vee) \ar[d]^{\cong \eqref{EqBoxtimesIsTensorFunctor}} \\
&&&&  \mf{X}\otimes \mf{X}^\vee
 }
 \]
and
\[
\xymatrix{
\mf{X}\otimes\mf{X}^\vee \ar[d]_{\eqref{EqBoxtimesIsTensorFunctor}\cong} \ar[drrrr]^{\ev_{\mf{X}}} &&&&\\
(\mf{X}_1^\vee \otimes \mf{X}_1)\boxtimes_{\mf{T}\otimes\mf{T}^\vee} (\mf{X}_2^\vee\otimes\mf{X}_2) \ar[rrrr]_{\ev_{\mf{X}_1}\boxtimes_{\ev_{\mf{T}}} \ev_{\mf{X}_2}} &&&& 1_{\BCoCorr_S} 
}
\]
Then $\mf{X}^\vee$, $\coev_{\mf{X}}$ and $\ev_{\mf{X}}$ witness the dualizability of $\mf{X}$.  It follows that $\mc{S}(\mf{X})=(X_1\times_T X_2,A_1\boxtimes_T A_2)$ is dualizable, so that $A_1\boxtimes_T A_2$ is ULA over $S$.   Now consider $\tr(1_{\mf{X}})=\ev_{\mf{X}}\circ \coev_{\mf{X}}$, an endomorphism of $1_{\BCoCorr_S}$.   On the one hand, $\mc{S}(\tr(1_{\mf{X}}))=\tr(1_{\mc{S}(\mf{X})})\in \End 1_{\CoCorr_S}$ is the data of the inertia stack $\In_S(X_1\times_T X_2)$ together with the characteristic class $\cc_{X_1\times_T X_2/S}(A)\in H^0(\In_S(X_1\times_T X_2),K_{\In_S(X_1\times_T X_2)/S})$.  On the other hand, \eqref{EqBoxtimesIsFunctorial} gives a 2-isomorphism
\[ \tr(1_{\mf{X}}) \isom (\ev_{\mf{X}_1}\boxtimes_{\ev_{\mf{T}}} \ev_{\mf{X}_2}) \circ (\coev_{\mf{X}_1}\boxtimes_{\coev_{\mf{T}}} \coev_{\mf{X}_2}) 
\isom \tr(1_{\mf{X_1}}) \boxtimes_{\tr(1_{\mf{T}})} \tr(1_{\mf{X}_2}).  \]
The source of this morphism is the correspondence $\In_S(X_1)\times_{\In_S(T_1)} \In_S(X_2)\to S\times_S S \isom S$ together with a global section of $K_{\In_S(X_1\times_T X_2)/S}$.  Reviewing the definition of $\boxtimes$ for morphisms in $\BCoCorr_S$ as in \eqref{EqFiberProductOfCorrespondences}, we see that this section is the image of $\cc_{X_1/S}(A_1)\otimes \cc_{X_2/S}(A_2)$ under 
\begin{eqnarray*}
 K_{\In_S(X_1)/S}\boxtimes_{\In_S(T)} K_{\In_S(X_2)/S} &\stackrel{\kappa_{\In_S(T)/S}}{\to}&
K_{\In_S(X_1\times_T X_2)/S} \otimes \In(p)^*K_{\In_S(T)} \\
&\isom& K_{\In_S(X_1\times_T X_2)/S}, 
\end{eqnarray*}
where the last isomorphism is induced from the inverse to 
$\cc_{T/S}(\Lambda_T)\from \Lambda_{\In_S(T)}  \to K_{\In_S(T)/S}$.  The result is exactly $\cc_{X_1/S}(A_1)\boxtimes_{\In_S(T)} \cc_{X_2/S}(A_2)$ as defined in Theorem \ref{ThmKunnethForCharacteristicClass}.


\subsection{The case of $[X/G]$ for $G$ smooth}

Let $X$ be a nice diamond over $S=\mathrm{Spd} C$ which is equipped with
an action of a cohomologically smooth $S$-group diamond $G$.   Let $\alpha\from X\times_S G\to X$ be the action map $(x,g)\mapsto g(x)$.   Let $Y=[X/G]$ be the stacky quotient;  this is an $S$-Artin v-stack which is locally nice over $S$.

Let $A\in D_{\mathrm{\acute{e}t}}(Y,\Lambda)$
be ULA over $S$.  Then the pair $(Y,A)$ is dualizable in $\CoCorr_S$,  and we obtain
a characteristic class 
\[
\mathrm{cc}_{Y/S}(A)\in H^{0}(\mathrm{In}_{S}(Y),K_{\mathrm{In}_{S}(Y)/S}).
\]
On the other hand,  the pullback $A_X$ of $A$ along $X\to Y$ is also ULA over $S$ (because $G\to S$ is cohomologically smooth).  For each element $g\in G(S)$,  we have an isomorphism $u_g\from A_X\to g^*A_X$ lying over $g\from X\to X$, The pair $(g,u_g)$ constitutes an endomorphism of the dualizable object $(X,A_X)$ in $\CoCorr_S$, so we may define the categorical trace $\tr(g,u_g)\in H^0(\Fix(g),K_{\Fix(g)/S})$.  Here $\Fix(g)=X\times_{g,X\times_S X,\Delta_{X/S}} X$ is the fixed-point locus of $g$ on $X$.  The object of this section is to show how the $\tr(g,u_g)$ can be derived from $\mathrm{cc}_{Y/S}(A)$.


First we give a concrete presentation of $\mathrm{In}_{S}(Y)$.   Define a correspondence $c$ on $X$ by
\begin{eqnarray*}
c=\pr_X\times_S \alpha:X\times_S G&\to& X\times_S X\\
(x,g)&\mapsto& (x,g(x)).
\end{eqnarray*}
Then the fixed-point locus $\Fix(c)\subset X\times_S G$ is $G$-stable for the $G$-action on $X\times_S G$ given by $h(x,g)=(h(x),hgh^{-1})$,  and then $\In_S(Y)\isom [\Fix(c)/G]$.  With respect to this isomorphism, the canonical map $p\from \In_S(Y)\to \In_S([S/G])\isom [G\sslash G]$ is the quotient by $G$ of the projection map $\Fix(c)\to G$.  

The $G$-equivariance of $A\vert_X$ may be expressed an isomorphism $u\from  A\vert_{X\times G} \to \alpha^*A\vert_X$.  This is not a cohomological correspondence in general (as $\alpha^*\neq \alpha^!$).   To obtain a cohomological correspondence on non-stacky objects,  we work over the base $G$.  Let $X_G=X\times_S G$,  and consider the correspondence $\tilde{c}$ defined by the diagram of diamonds over $G$:
\[
\xymatrix{ 
& X_G \ar[dl]_{\id_{X_G}} \ar[dr]^{\tilde{\alpha}\from (x,g)\mapsto (g(x),g) } & \\
X_G && X_G
}
\]
By design,  the fiber of this correspondence over $g\in G(C)$ is the graph of the automorphism $g\from X\to X$.  
Moreover, there is a natural isomorphism $\Fix(c)\isom\Fix(\tilde{c})$, and the fiber of $\mathrm{Fix}(\tilde{c})$ over any $g\in G(C)$
is exactly $\mathrm{Fix}(g)$.  
The $G$-equivariance of $A\vert_{X}$ is encoded by an isomorphism $\tilde{u}\from A\vert_{X_G}\to \tilde{\alpha}^*A\vert_{X_G}$.  Since $\tilde{\alpha}$ is an isomorphism, we have $\tilde{\alpha}^*\isom\tilde{\alpha}^!$,  and therefore the pair $(\tilde{c},\tilde{u})$ constitutes an endomorphism of the dualizable object $(X_G,A\vert_{X_G})$ of $\CoCorr_G$.  The categorical trace of $(\tilde{c},\tilde{u})$ is an element
\[\tr(\tilde{c},\tilde{u}) \in H^0(\Fix(\tilde{c}),K_{\Fix(\tilde{c})/G}). \]
This is the ``universal local term'' for the action of $G$ on $X$,  in the sense that for any $g\in G(C)$, the restriction map
\[ H^0(\Fix(\tilde{c}),K_{\Fix(\tilde{c})/G}) \to H^0(\Fix(g), K_{\Fix(g)/S}) \]
carries $\tr(\tilde{c},\tilde{u})$ onto $\tr(g,u_g)$.   

We want to compare the characteristic class $\mathrm{cc}_{Y/S}(A)$
with the universal local term $\tr(\tilde{c},\tilde{u})$.
To do this, we first observe that from the Cartesian square
\[
\xymatrix{\mathrm{Fix}(\tilde{c})\ar[d]_{q}\ar[r] & G\ar[d]\\
\mathrm{In}_{S}(Y)\ar[r] & [G\sslash G]
}
\]
we obtain a canonical map $q^{\ast}K_{\mathrm{In}_{S}(Y)/[G\sslash G]}\to K_{\mathrm{Fix}(\tilde{c})/G}$,
and thus a canonical pullback map
\begin{equation}
\label{EqPullbackMap}
q^*\from H^{0}(\mathrm{In}_{S}(Y),K_{\mathrm{In}_{S}(Y)/[G\sslash G]})\to H^{0}(\mathrm{Fix}(\tilde{c}),K_{\mathrm{Fix}(\tilde{c})/G}).
\end{equation}
Next,  Lemma \ref{LemTrivialDualizingSheaf} applied to $T=[S/G]$ shows that $\cc_{T/S}(\Lambda_T)$ is an isomorphism $\Lambda_{[G\sslash G]} \isomto K_{[G\sslash G]/S}$.  This induces an isomorphism
\begin{equation}
\label{EqIdentificationOfDualizingSheaves}
K_{\In_S(Y)/[G\sslash G]} \isom p^!\Lambda_{[G\sslash G]} \isomto p^!K_{[G\sslash G]/S} \isom 
K_{\In_S(Y)/S}. 
\end{equation}
 
Combining \eqref{EqPullbackMap} and \eqref{EqIdentificationOfDualizingSheaves}, we obtain a canonical map
\begin{equation}
\label{EqDefinitionOfIota}
\iota:H^{0}(\mathrm{In}_{S}(Y),K_{\mathrm{In}_{S}(Y)/S})\to H^{0}(\mathrm{Fix}(\tilde{c}),K_{\mathrm{Fix}(\tilde{c})/G}).
\end{equation}
The main result of this section is the following theorem.
\begin{thm}
\label{ThmCharClassOnXModG}
Notation and assumptions as above, we have an equality
\[
\iota\left(\mathrm{cc}_{Y/S}(A)\right)=\mathrm{tr}_{\tilde{c}}(\tilde{u},A|_{X_{G}}).
\]
\end{thm}

\begin{proof}  We restate the theorem in the language of based cohomological correspondences.  The main players are
\begin{itemize}
\item $T=([S/G],\Lambda_{[S/G]})$, a dualizable object of $\CoCorr_S$.
\item $\mf{Y}=(Y\to [S/G],A,\Lambda_{[S/G]})$, a dualizable object of $\BCoCorr_S$ with base $T$.
\item $\mf{X}_G=(X_G,A_{X_G})$, a dualizable object of $\CoCorr_G$ with base $1_{\CoCorr_G}$.
\item $\alpha\in \End \mf{X}_G$, the endomorphism described by the pair $(\tilde{c},\tilde{u})$.
\end{itemize}
We would like to relate $\tr(\id_{\mf{Y}})$ to $\tr(\alpha)$.  The idea is to promote $\alpha$ to an endomorphism of based cohomological correspondences which lies over $\id_{T}$.  To this end we introduce some more objects in $\BCoCorr_S$:
\begin{itemize}
\item $\mf{G}=(G\to S,\Lambda_G,\Lambda_S)$ with base $1_{\CoCorr_S}$,
\item $\mf{G}'=(G\to [S/G]\times_S [S/G],\Lambda_G,\Lambda_{[S/G]}\boxtimes_S K_{[S/G]/S})$, with base $T\otimes T^\vee$, where the morphism $G\to [S/G]\times_S [S/G]$ is defined as the trivial $G\times_S G$-torsor $G_{G\times_S G}=G\times_S G\times_S G$.
\end{itemize}
We also define morphisms in $\BCoCorr_S$:
\begin{itemize}
\item $\coev_G \from \mf{G}\to \mf{G}'$, which has base $\coev_T$ and source $1_{(G,\Lambda_G)}$,
\item $\ev_G\from \mf{G}'\to \mf{G}$, which has base $\ev_T$ and source $1_{(G,\Lambda_G)}$.
\item An endomorphism $\alpha_0\from \mf{G}'\to \mf{G}'$ lying over $\id_{T\otimes T^\vee}$, corresponding\footnote{Strictly speaking, v-stacks form a 2-category, and we are describing here a 2-morphism from $G\to [S/G]^2$ to itself.}to the automorphism $G_{G\times G}\to G_{G\times G}$ defined by $(x,g,h)\mapsto (x,gx,h)$.  
\end{itemize}
Now observe that $\tr_G(\alpha_0):=\ev_G\circ\alpha_0\circ\coev_G$ is an endomorphism of $\mf{G}$ with base $\tr(\id_T)$ and source $\id_{\mc{S}}(\mf{G})$, whose underlying based correspondence is shown in the diagram:
\[
\xymatrix{
G \ar[d] & G \ar[l]_{\id_G} \ar[d] \ar[r]^{\id_G} & G \ar[d] \\
S & [G\sslash G] \ar[l] \ar[r] & S
}
\]
where the central horizontal arrow sends $g$ to its own conjugacy class.  

Recall that $\mc{S}\from \BCoCorr_S\to \CoCorr_S$ takes a based cohomological corresponce onto its source.  Let $\mc{F}\from \CoCorr_G\to\CoCorr_S$ be the functor which forgets the base $G$.  We have a diagram in $\CoCorr_S$:
\[
\xymatrix{
\mc{S}(1_{\BCoCorr_S} \boxtimes_{1_{\CoCorr_S}}\mf{G}) 
\ar[d]_{\mc{S}(\coev_{\mf{Y}}\boxtimes_{\coev_T} \coev_G)} 
\ar[rr]^{\sim} 
&&
\mc{F}(1_{\CoCorr_G})
\ar[d]^{\mc{F}(\coev_{\mf{X}_G})} 
\\
\mc{S}((\mf{Y}\otimes\mf{Y}^\vee) \boxtimes_{T\otimes T^\vee} \mf{G}')
\ar[d]_{\mc{S}(\id_{\mf{Y}\otimes \mf{Y}^\vee}  \boxtimes_{\id_{T\otimes T^\vee}} \alpha_0)} 
\ar[rr]^{\sim}
&&
\mc{F}(\mf{X}_G \otimes \mf{X}_G^\vee)
\ar[d]^{\mc{F}(\alpha)} 
\\
\mc{S}((\mf{Y}\otimes\mf{Y}^\vee) \boxtimes_{T\otimes T^\vee} \mf{G}') 
\ar[d]_{\mc{S}(\ev_{\mf{Y}} \boxtimes_{\ev_T} \ev_G )}
\ar[rr]^{\sim}
&&
\mc{F}(\mf{X}_G\otimes \mf{X}_G^\vee) 
\ar[d]^{\mc{F}(\ev_{\mf{X}_G})}
\\
\mc{S}(1_{\BCoCorr_S} \boxtimes_{1_{\CoCorr_S}} \mf{G})
\ar[rr]^{\sim}
&&
\mc{F}(1_{\CoCorr_G})
}
\]
where all squares are filled in with 2-isomorpisms.  The functoriality property of $\boxtimes$ from \eqref{EqBoxtimesIsFunctorial} now gives a 2-isomorphism
\begin{equation}
\label{EqCompareCCToTrace}
 \mc{S}\left(\cc_{Y/S}(A)\boxtimes_{\cc_{[S/G]/S}(\Lambda_{[S/G]})}  \tr_G(\alpha_0) \right)\isomto \mc{F}(\tr(\alpha)). 
 \end{equation}
The isomorphism of v-stacks implicit in \eqref{EqCompareCCToTrace} is expressed by the fact that we have a cartesian diagram:
\[
\xymatrix{
\Fix(\tilde{c}) \ar[r] \ar[d] & G \ar[d] \\
\In_S(Y) \ar[r] & [G\sslash G] 
}
\]
On the level of cohomology classes, \eqref{EqCompareCCToTrace} tells us that $\tr(\alpha)$, considered as an element of $H^0(\Fix(\tilde{c}),K_{\Fix(\tilde{c})/S})$ can be derived from $\cc_{Y/S}(A)$ in the manner described by the theorem.
\end{proof}

We conclude the section with a remark about isolated fixed points.  Assume there exists a conjugacy-invariant open subset $U\subset G$ whose elements act on $X$ with only isolated fixed points.  (This is the case for the action of the positive loop group on the affine Grassmannian. We study that scenario in the next section.)   Write $\In_S([X/G])_U$ for the pullback of $[U\sslash G]$ under $\In_S([X/G])\to [G\sslash G]$.  Then $\In_S([X/G])_U\to [U\sslash G]$ is \'etale over $[U\sslash G]$;  as such we have a canonical trivialization $K_{\In_S([X/G]_U/S}\isom \Lambda_{\In_S([X/G])_U}$.  Therefore the restriction over $U$ of the characteristic class of $A$ is an element
\[ cc_{[X/G]/S}(A)^U\in H^0(\In_S([X/G])_U,\Lambda); \]
that is, it is a continuous function on the space of pairs $(x,g)\in X\times_S U$ with $g(x)=x$.  Theorem \ref{ThmCharClassOnXModG} implies that this function is $(x,g)\mapsto \loc_x(g,A)$.




